Emergence of Metcalfe's Law: Mechanism and Model

Metcalfe's Law captures the relationship between the value of a network and its scale, asserting that a network's value is directly proportional to the square of its size. Over the past four decades, various researchers have proposed different scaling laws on this subject. Remarkably, these seemingly conflicting conclusions have all been substantiated by robust data validation, raising the question of which law holds greater representativeness. Consequently, there remains a need for inherent mechanism to underpin these laws. This study aims to bridge this disparity by offering a theoretical interpretation of Metcalfe's Law and its variations. Based on a certain degree of consensus that "traffic is value", network effects are gauged using network traffic load. A general analytical boundary for network traffic load is deduced by balancing practicality and analytical feasibility through the establishment of a comprehensive network model. From this foundation, the mechanism behind Metcalfe's Law and its variants is elucidated, aligning the theoretical derivations with the previously validated empirical evidence for Metcalfe's Law.

==> analysis.tex <==
\subsection*{Theoretical Analysis}
In this section, we delve into a detailed analysis of traffic load quantification in the network. We present a comprehensive model that allows us to quantify the traffic load and derive meaningful insights. To validate our findings, we provide a proof to support the conclusions.

\subsection*{Basic Lemma to Derive the Traffic Load}


\begin{lem}[Minimal Spanning Tree \cite{steele1988growth}]\label{lem-growthsteel}
	Let $X_i$, $1\leq i <\infty$, denote independent random variables with
	values in $\mathbb{R}^d$, $d\geq 2$, and let $M_n$ denote the cost of
	a minimal spanning tree of a complete graph with vertex set $\{X_i\}_{i=1}^n$, where the cost of an edge $(X_i, X_j)$ is given by $\Psi((|X_i-X_j|))$.
	Here, $|X_i-X_j|$ denotes the Euclidean distance between $X_i$ and $X_j$ and
	$\Psi$ is a monotone function. For bounded random variables and $0<\sigma<d$,
	it holds that as $n\to \infty$, with probability $1$, one has
	\[
	M_n\sim c_1(\sigma,d)\cdot n^{\frac{d-\sigma}{d}} \cdot \int_{\mathbb{R}^d}f(X)^{\frac{d-\sigma}{d}}d X,\]
	%\footnote{For two functions $g_1(n)$ and $g_2(n)$, we say $g_1(n)\sim g_2(n)$ if and only if
		%$\lim_{n\to \infty} {g_1(n)}/{g_2(n)}=1$.}
	provided $\Psi(x)\sim x^\sigma$, where $f(X)$ is the density of the absolutely continuous part of the distribution of the $\{X_i\}$.
\end{lem}

\begin{lem}[Kolmogorov's Strong LLN \cite{williams1991probability}]\label{lem-Kolmogorov-slln}
	Let $\{X_n\}$  be an i.i.d. sequence of random variables having finite mean: For $\forall n$,
	$\mathbb{E}[X_n] < \infty$.
	Then, a strong law of large numbers (LLN) applies to the sample mean:
	\[\bar{X}_n \stackrel{a.s.}{\longrightarrow} \mathbb{E}[X_n],\]
	where  $\stackrel{a.s.}{\longrightarrow}$ denotes \emph{almost sure convergence}.
\end{lem}

\begin{lem}\label{basic_lemma_emst} For $k=1,2,\cdots,n$, it holds that
	\begin{equation*}
		\begin{aligned}
			\mathrm{L}_{\mathrm{N}}^{\ast}= \lambda \cdot\Omega\left( \sum_{k=1}^{n}|\EMST(\{u_{k}\}\cup \mathbb{D}_{k})|\right),
		\end{aligned}
	\end{equation*}
	where $\EMST(\cdot)$ denotes the Euclidean minimum spanning tree over a set.
	
\end{lem}

See Lemma 1 of \cite{mobihoc2014} for the proof of this lemma.

\begin{lem}\label{lem-Pr}
	Consider the Zipf's distribution whose distribution function like $\Pr(q_k=q)={\left(\sum\nolimits_{j=1}^{n-1}j^{-\alpha}\right)^{-1}} \cdot {q^{-\alpha}}$, where $\alpha$ is a parameter to describe the distribution, we get that
	\begin{equation}\label{eq-Pr}
	\Pr(q_k=q)= \left\{
		\begin{array}{ll}
			\Theta\left( q^{-\alpha} \right)  , &  \alpha>1;  \\
			\Theta\left(\frac{1}{\log n}\cdot q^{-1}  \right), &  \alpha=1;  \\
			\Theta\left(n^{\alpha-1}\cdot q^{-\alpha} \right)  , & 0< \alpha< 1.
		\end{array}
		\right.
	\end{equation}
	\end{lem}


\begin{table*}[!t]
	\vspace{-0.3in}
	\renewcommand{\arraystretch}{1.45}
	\centering
	\caption{\centering The Results on the Traffic Load $\mathrm{L}_{\mathrm{N}}^{\ast}$ and Labeling of Scaling Laws under $\lambda=\Theta(1)$}
	\label{G-tab-total}
	\resizebox{0.9\linewidth}{!}
	{
		%\begin{tiny}
		\begin{tabular}{ !{\vrule width1.2pt} l!{\vrule width1.2pt}c|c|c|c|c !{\vrule width1.2pt} }
			
			
			\toprule
			$\mathcal{d}$ $\backslash$ $\mathcal{s}$ & $\mathcal{s}>2$ & $\mathcal{s}=2$ & $ 1<\mathcal{s}<2 $ & $\mathcal{s}=1$ & $0\leq\mathcal{s}<1$ \\
			\toprule
			% \midrule
			
			
			$\mathcal{d}>2$ &
			\makeatletter
			\newtcolorbox{tcbmath}[2][]{
				ams #2,
				% expanding `size=small`
				boxrule=0pt, boxsep=0pt,
				left=0pt, right=0pt, top=.5ex, bottom=.5ex,
				toptitle=0pt, bottomtitle=0pt,
				% middle=0.5mm, % optional
				arc=0pt,
				colback=cyan!80!black!50
			}
			
			\tcbset{
				highlight math style={
					size=small,
					colframe=white,
					colback=blue!10!white
				}
			}
			\makeatother
			
			% \tcbhighmath{\lambda \cdot \Omega(n)},\\
			$\tcbhighmath{\lambda \cdot \Omega(n)} , \mathcal{i}\geq0. $ &
			\makeatletter
			\newtcolorbox{tcbmath}[2][]{
				ams #2,
				% expanding `size=small`
				boxrule=0pt, boxsep=0pt,
				left=0pt, right=0pt, top=.5ex, bottom=.5ex,
				toptitle=0pt, bottomtitle=0pt,
				% middle=0.5mm, % optional
				arc=0pt,
				colback=cyan!80!black!50
			}
			
			\tcbset{
				highlight math style={
					size=small,
					colframe=white,
					colback=green!10!white
				}
			}
			\makeatother
			
			% \tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
			$ \tcbhighmath{\lambda \cdot \Omega(n \log n)} , \mathcal{i}\geq0. $ &
			$ \lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}}) , \mathcal{i}\geq0. $ &
			$ \lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n}), \mathcal{i}\geq0. $ &
			
			$ \lambda \cdot \Omega(n^{\frac{3}{2}}), \mathcal{i}\geq0. $ \\
			\midrule
			
			$\mathcal{d}=2$ & $\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				% \uline{\lambda \cdot \Omega(n)}  , \\
				\qquad   \mathcal{i} >1;\\
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				%\dashuline{\lambda \cdot \Omega(n \log n)} ,  \\
				%\qquad \mathcal{i}=1;  \\
				%\Omega(n \cdot \log n)  , \\
				\qquad 0\leq\mathcal{i}\leq1.\\
			\end{array}
			\right. $ &
			
			\makeatletter
			\newtcolorbox{tcbmath}[2][]{
				ams #2,
				% expanding `size=small`
				boxrule=0pt, boxsep=0pt,
				left=0pt, right=0pt, top=.5ex, bottom=.5ex,
				toptitle=0pt, bottomtitle=0pt,
				% middle=0.5mm, % optional
				arc=0pt,
				colback=cyan!80!black!50
			}
			
			\tcbset{
				highlight math style={
					size=small,
					colframe=white,
					colback=green!10!white
				}
			}
			\makeatother
			
			
			$ \tcbhighmath{\lambda \cdot \Omega(n \log n)}$  ,  $ \mathcal{i}\geq0. $  &
			$ \lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}})  ,  \mathcal{i}\geq0. $  &
			$ \lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n}) $ , $ \mathcal{i}\geq0. $ &
			
			$ \lambda \cdot \Omega(n^{\frac{3}{2}}) ,  \mathcal{i}\geq0. $  \\
			\midrule
			
			$\frac{3}{2}<\mathcal{d}<2$ & $\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				% \uline{\lambda \cdot \Omega(n)} , \\
				\qquad  \mathcal{i}>3-\mathcal{d};  \\
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)} , \\
				\qquad  \mathcal{i}=3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}})  , \\
				\qquad  1<\mathcal{i}<3-\mathcal{d}; \\
				\lambda \cdot \Omega( n^{3-\mathcal{d}} / \log n) , \\
				\qquad  \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  , \\
				\qquad  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n  \log n)} , \\
				\qquad  \mathcal{i}\geq3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}})  , \\
				\qquad  1<\mathcal{i}<3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad  \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  , \\
				\qquad  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}}) , \\
				\qquad  \mathcal{i}\geq3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}})  , \\
				\qquad  1<\mathcal{i}<3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad  \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  , \\
				\qquad  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ &
			%$\left\{
			%  \begin{array}{ll}
				%\Omega(n^{\frac{3}{2}} / \sqrt{\log n}) , \\
				%\qquad  \mathcal{i}>1; \\
				%\Omega(n^{\frac{3}{2}} / \sqrt{\log n}) , \\
				%\qquad  \mathcal{i}=1; \\
				
				
				$\lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n}) ,   \mathcal{i}\geq0. $ &
				%  \end{array}
			%\right. $
			%\left\{
			%  \begin{array}{ll}
				%\Omega(n^{\frac{3}{2}}) , \\
				%\qquad  \mathcal{i}>1; \\
				%\Omega(n^{\frac{3}{2}}) , \\
				%\qquad  \mathcal{i}=1; \\
				$\lambda \cdot \Omega(n^{\frac{3}{2}}),  \mathcal{i}\geq0. $ \\
				%  \end{array}
			%\right. $ \\
			\midrule
			
			$\mathcal{d}=\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				
				% \uline{\lambda \cdot \Omega(n)}  ,   \\
				\qquad \mathcal{i} >\frac{3}{2};\\
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)} , \\
				\qquad \mathcal{i}=\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{\frac{5}{2}-\mathcal{i}}) , \\
				\qquad 1<\mathcal{i}<\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \log n) , \\
				\qquad \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}})  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)}  ,   \\
				\qquad \mathcal{i} \geq\frac{3}{2};\\
				\lambda \cdot \Omega(n^{\frac{5}{2}-\mathcal{i}}) , \\
				\qquad 1<\mathcal{i}<\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \log n) , \\
				\qquad \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}})  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}})  ,   \\
				\qquad  \mathcal{i} \geq\frac{3}{2};\\
				\lambda \cdot \Omega(n^{\frac{5}{2}-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \log n) , \\
				\qquad \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{\frac{3}{2}})  ,  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad  \mathcal{i} >1;\\
				%\Omega(n^{\frac{3}{2}} \cdot \sqrt{\log n})  ,  \\
				%\qquad \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \sqrt{\log n})  ,  \\
				\qquad  0\leq\mathcal{i}\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}}),   \\
				\qquad  \mathcal{i} >1;\\
				%\Omega(n^{\frac{3}{2}} \cdot \log n)  ,  \\
				%\qquad \mathcal{i}=1;\\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \log n)  ,  \\
				\qquad  0\leq\mathcal{i}\leq1.\\
			\end{array}
			\right. $ \\
			\midrule
			
			$1<\mathcal{d}<\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				
				% \uline{\lambda \cdot \Omega(n)}  ,  \\
				\qquad  \mathcal{i}>3-\mathcal{d}; \\
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)} , \\
				\qquad \mathcal{i}=3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}}) , \\
				\qquad  1<\mathcal{i}<3-\mathcal{d};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad  \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)}  ,  \\
				\qquad \mathcal{i}\geq3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}}) , \\
				\qquad 1<\mathcal{i}<3-\mathcal{d};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  ,  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}})  ,  \\
				\qquad  \mathcal{i}\geq3-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}}) , \\
				\qquad  1<\mathcal{i}<3-\mathcal{d};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad  \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,  \\
				\qquad \mathcal{i}>\frac{5}{2}-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \sqrt{\log n}) , \\
				\qquad \mathcal{i}=\frac{5}{2}-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}}) , \\
				\qquad 1<\mathcal{i}<\frac{5}{2}-\mathcal{d};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				
				\lambda \cdot \Omega(n^{\frac{3}{2}}),  \\
				\qquad \mathcal{i}>\frac{5}{2}-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \cdot \log n) , \\
				\qquad \mathcal{i}=\frac{5}{2}-\mathcal{d}; \\
				\lambda \cdot \Omega(n^{4-\mathcal{i}-\mathcal{d}}) , \\
				\qquad 1<\mathcal{i}<\frac{5}{2}-\mathcal{d};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}} / \log n) , \\
				\qquad \mathcal{i}=1; \\
				\lambda \cdot \Omega(n^{3-\mathcal{d}})  ,  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ \\
			\midrule
			
			$\mathcal{d}=1$ & $\left\{
			\begin{array}{ll}
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				% \uline{\lambda \cdot \Omega(n)}  ,   \\
				\qquad  \mathcal{i}\geq 2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}} / \log n) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / (\log n)^2) , \\
				\qquad  \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{2} / \log n)  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)}  ,   \\
				\qquad \mathcal{i}\geq 2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}} / \log n) , \\
				\qquad 1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / (\log n)^2) , \\
				\qquad  \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{2} / \log n)  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}})  ,   \\
				\qquad \mathcal{i}\geq 2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}} / \log n) , \\
				\qquad 1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / (\log n)^2) , \\
				\qquad  \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{2} / \log n)  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad \mathcal{i}\geq 2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}} / \log n) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / (\log n)^2) , \\
				\qquad  \mathcal{i}=1;  \\
				\lambda \cdot \Omega(n^{2} / \log n)  ,  \\
				\qquad 0\leq\mathcal{i}<1.\\
				
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				
				\lambda \cdot \Omega(n^{\frac{3}{2}}),   \\
				\qquad \mathcal{i}\geq 2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}} / \log n) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / (\log n)^2) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!25!white
					}
				}
				\makeatother
				
				\lambda \cdot \Omega(n^{2} / \log n)  ,  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$0\leq\mathcal{d}<1$ & $\left\{
			\begin{array}{ll}
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=blue!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n)},\\
				% \uline{\lambda \cdot \Omega(n)}  ,   \\
				\qquad  \mathcal{i}>2;\\
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				% \dashuline{\lambda \cdot \Omega(n \log n)} , \\
				\qquad  \mathcal{i}=2;  \\
				\lambda \cdot \Omega(n^{3-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / \log n) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!45!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n^{2})}, \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=green!10!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n \log n)},\\
				%\dashuline{\lambda \cdot \Omega(n \log n)}  ,   \\
				\qquad  \mathcal{i}\geq2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / \log n) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!45!white
					}
				}
				\makeatother
				
				\tcbhighmath{ \lambda \cdot \Omega(n^{2})},  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{2-\frac{\mathcal{s}}{2}})  ,   \\
				\qquad \mathcal{i}\geq2;\\
				\lambda \cdot \Omega(n^{3-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<2;  \\
				\lambda \cdot \Omega(n^{2} / \log n) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!45!white
					}
				}
				\makeatother
				
				\tcbhighmath{ \lambda \cdot \Omega(n^{2})}, \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad  \mathcal{i}>\frac{3}{2};\\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \sqrt{\log n}) , \\
				\qquad  \mathcal{i}=\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{2} / \log n) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!45!white
					}
				}
				\makeatother
				
				\tcbhighmath{ \lambda \cdot \Omega(n^{2})},  \\
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\lambda \cdot \Omega(n^{\frac{3}{2}}),   \\
				\qquad  \mathcal{i}>\frac{3}{2};\\
				\lambda \cdot \Omega(n^{\frac{3}{2}} \cdot \log n) , \\
				\qquad  \mathcal{i}=\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{3-\mathcal{i}}) , \\
				\qquad  1<\mathcal{i}<\frac{3}{2};  \\
				\lambda \cdot \Omega(n^{2} / \log n) , \\
				\qquad  \mathcal{i}=1;  \\
				
				\makeatletter
				\newtcolorbox{tcbmath}[2][]{
					ams #2,
					% expanding `size=small`
					boxrule=0pt, boxsep=0pt,
					left=0pt, right=0pt, top=.5ex, bottom=.5ex,
					toptitle=0pt, bottomtitle=0pt,
					% middle=0.5mm, % optional
					arc=0pt,
					colback=cyan!80!black!50
				}
				
				\tcbset{
					highlight math style={
						size=small,
						colframe=white,
						colback=yellow!45!white
					}
				}
				\makeatother
				
				\tcbhighmath{\lambda \cdot \Omega(n^{2})},  \\
				
				
				\qquad  0\leq\mathcal{i}<1.\\
			\end{array}
			\right. $ \\
			\bottomrule
			\multicolumn{6}{c}{
				
				
				\begin{Metcalfe}
					\qquad
				\end{Metcalfe}
			 \textbf{Metcalfe's Law}\quad 
				\begin{Sarnoff}
					\qquad
				\end{Sarnoff}
				 \textbf{Sarnoff's Law}\quad
				\begin{Odlyzko}
					\qquad
				\end{Odlyzko}
				 \textbf{Odlyzko's Law}\quad 
				
				When $\lambda=\Theta(1)$, \textbf{cube law} cannot be achieved.
				
			}
		\end{tabular}
		%\end{tiny}
		%\vspace{-15cm}
	}
\end{table*}

\subsection*{Euclidean Minimum Spanning Tree}
Denote a network session by an ordered pair $\mathrm{T}_k=<v_{k}, \mathcal{A}_k>$, where $ v_{k} $ is the source and each element $ v_{k_{i}} $ in $\mathcal{A}_k=\{v_{k_i}\}_{i=1}^{r_k}$ is the nearest node to the corresponding $ p_{k_{i}} $ in $ \mathcal{d}^\mathrm{I}_k=\{p_{k_i}\}_{i=1}^{r_k} $, the random variable $r_{k}$ denotes the number of potential destinations for session $\mathrm{T}_k$, i.e.,
The destination for node $v_k$ is dynamically selected based on the data being transported within the network during the session. % the friends of $v_{k}$ who are interested in the message from $v_{k}$ in this session.
We call point $p_{k_{i}}$ the \emph{anchor point} of $v_{k_{i}}$, and define a set $\mathcal{P}_{k} := \{v_{k}\} \cup \mathcal{A}_k$. Then, we can get the following lemma.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}\label{lem-EMST-B-D} For a network broadcast session $\mathrm{T}_k$, when $ r_{k}=\omega(1) $, with probability $1$, it holds that
	\begin{equation*}
		|\EMST(\mathcal{A}_k)|=\Theta(L_{\mathcal{P}}(\mathcal{s}, r_k)),
	\end{equation*}
	and then
	\begin{equation*}
		|\EMST(\mathcal{P}_{k})|=\Omega(L_{\mathcal{P}}(\mathcal{s}, r_k)),
	\end{equation*}
	where $\EMST(\cdot)$ denotes the Euclidean minimum spanning tree over a set,
	\begin{equation}\label{eq-L-P-beta-9765}
		L_{\mathcal{P}}(\mathcal{s}, r_k) = \left\{
		\begin{array}{ll}
			\Theta\left( \sqrt{r_k} \right)  , &  \mathcal{s}>2;  \\
			\Theta\left(\sqrt{r_k} \cdot \log n  \right), &  \mathcal{s}=2;  \\
			\Theta\left(\sqrt{r_k} \cdot n^{1-\frac{\mathcal{s}}{2}} \right)  , & 1< \mathcal{s} < 2;  \\
			\Theta\left(\sqrt{r_k} \cdot \sqrt{\frac{n}{\log n}} \right) , &  \mathcal{s}=1;  \\
			\Theta\left(\sqrt{r_k} \cdot \sqrt{n} \right)  , &  0\leq\mathcal{s} <1.
		\end{array}
		\right.
	\end{equation}
%	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{lem}


% \subsection{Proof of Lemma \ref{lem-EMST-B-D}}\label{proof-lem-EMST-B-D}
\begin{proof}
	With probability $1$, it holds that
	\begin{center}
		$	|\EMST(\mathcal{A}_k)|=\Theta(L_{\mathcal{P}}(\mathcal{s}, r_k))$ for $r_k=\omega(1)$,
	\end{center}
	where $L_{\mathcal{P}}(\mathcal{s}, r_k)$ is defined in Eq.(\ref{eq-L-P-beta-9765}). Combining with the fact that \[|\EMST(\mathcal{P}_{k})|\geq |\EMST(\mathcal{A}_k)|,\] then, we get that
	\begin{equation*}
		|\EMST(\mathcal{P}_{k})|=\Omega(L_{\mathcal{P}}(\mathcal{s}, r_k)).
	\end{equation*}
	Then, our focus turns to the derivation of $ L_{\mathcal{P}}(\mathcal{s}, r_k) $. The  given $X_0$ is a point from $\mathcal{O}$ selected arbitrarily and make $X_0$ as the reference point. The distribution of points in $\mathcal{A}_k$ follows the density function
	\begin{equation*}
		f_{X_0}(X)=\frac{\left(\int_{\mathcal{D}(X_0,|X-X_0|)}\mathbf{d}(Y)dY+1\right)^{-s}}{\int_{\mathcal{O}}\left(\int_{\mathcal{D}(X_0,|X-X_0|)}\mathbf{d}(Y)dY+1\right)^{-s}dZ},
	\end{equation*}
	where 
	$\mathbf{d}(Y)=n\sum\nolimits_{c_j\in \mathcal{C}} \frac{g(|Y-c_j|)}{\int_{\mathcal{O}}g(|Z-c_j|)dZ}$ and $\mathcal{C}$ is the positions set of points from \cite{mobihoc2014}. 
	
	While we assume that $\mathcal{g}=0$, we get $g(\cdot)=1$ and $\mathbf{d}(Y)=1$. Combining the conclusion of Lemma \ref{lem-Pr}, the density function can be calculated as:
	\begin{equation*}\label{eq-g-f-X0-X}
		f_{X_0}(X) = \left\{
		\begin{array}{ll}
			\Theta\left( (|X-X_0|^2+1)^{-\mathcal{s}} \right)  , &  \mathcal{s}>1;  \\
			\Theta\left(\frac{1}{\log n}\cdot (|X-X_0|^2+1)^{-1}  \right), &  \mathcal{s}=1;  \\
			\Theta\left(n^{\mathcal{s}-1}\cdot(|X-X_0|^2+1)^{-\mathcal{s}} \right)  , & 0< \mathcal{s} < 1.
		\end{array}
		\right.
	\end{equation*}
	
	Based on the value of $\mathcal{s}$, we have:
	
	
	
%	
%	(1) When $ 0 \leq\beta <1 $,
%	\begin{equation*}
%		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)} dX =  \Theta\left(n^{\frac{\beta-1}{2}} \cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right)
%	\end{equation*}
%	$~~~~~~~~~~~~~~~~~~~~~~~= \Theta\left(n^{\frac{\beta-1}{2}} \cdot n^{1-\frac{\beta}{2}}\right) = \Theta\left(\sqrt{n}\right) $.
%	
%	
%	(2) When $ \beta=1 $,
%	\begin{equation*}
%		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left(\frac{1}{\sqrt{\log n}}\cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{1}{2}}}\right)
%	\end{equation*}
%	$~~~~~~~~~~~~~~~~~~~~~~~= \Theta\left(\frac{1}{\sqrt{\log n}} \cdot \sqrt{n}\right) = \Theta\left(\sqrt{\frac{n}{\log n}}\right) $.
%	
%	(3) When $ \beta>1 $,
%	\begin{equation*}
%		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right).
%	\end{equation*}
%	
%	Especially,
%	
%	when $ 1<\beta<2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right) = \Theta\left(n^{1-\frac{\beta}{2}}\right) $;
%	
%	when $ \beta=2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)}\right) $=$ \Theta\left(\log n\right) $;
%	
%	when $ \beta>2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right) $=$ \Theta\left(1\right) $.
	
		(1) When $ \mathcal{s}>1 $,
	\begin{equation*}
		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right)
	\end{equation*}
	\begin{equation*}
		%\Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right) 
		~~~~~~~~~~~~~~~~~~~~~~=\left\{
		\begin{array}{ll}
			\Theta\left(1\right) , & \mathcal{s}>2;\\
			\Theta\left(\log n\right) , & \mathcal{s}=2;\\
			\Theta\left(n^{1-\frac{\mathcal{s}}{2}}\right) , & 1<\mathcal{s}<2.
		\end{array}
		\right.
	\end{equation*}
	
	
	(2) When $ \mathcal{s}=1 $,
	\begin{equation*}
		\begin{aligned}
			\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX &= \Theta\left(\frac{1}{\sqrt{\log n}}\cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{1}{2}}}\right)\\
			& = \Theta\left(\sqrt{\frac{n}{\log n}}\right).
		\end{aligned}
	\end{equation*}
	
	(3) When $ 0 \leq\mathcal{s} <1 $,
	\begin{equation*}
		\begin{aligned}
			\int_{\mathcal{O}}\sqrt{f_{X_0}(X)} dX &=  \Theta\left(n^{\frac{\mathcal{s}-1}{2}} \cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right)\\
			&= \Theta\left(\sqrt{n}\right).
		\end{aligned}
	\end{equation*}
	
	Combining with all cases above, we complete the proof.$\hfill\square$
\end{proof}

\subsection{Main Results on Traffic Load}\label{Z-D-result-interestcast}
The following theorem demonstrates a theoretical bound on the traffic load for network $\mathrm{N}$ as follows.
\begin{thm}\label{Z-D-thm-traffic-load-on-sessions}
	Let $\mathrm{L}_{\mathrm{N}}^{\ast}$ denote the traffic load for data transportation in network $\mathrm{N}$ with $n$ nodes.
	It holds that
	\begin{equation*}
		% \mathrm{L}_{\mathbb{N}}=\lambda\cdot\Omega\left(G\left(\mathcal{i}, \mathcal{s}, \mathcal{d}\right)\right),
		\mathrm{L}_{\mathrm{N}}^{\ast}=\mathrm{L}_{\mathrm{N}}^{\ast}\left(\lambda,\mathcal{i},\mathcal{s},\mathcal{d},n\right),
	\end{equation*}
	where the value of $\mathrm{L}_{\mathrm{N}}$, presented in Table \ref{G-tab-total},
	% of our technical report \cite{dropboxmobihoc2016},
	depends on  the data arrival/generating rate $\lambda$, exponent of node influence distribution $\mathcal{i}$, exponent of relationship separation distribution $\mathcal{s}$ and exponent of data destination distribution $\mathcal{d}$.
	
\end{thm}

%v\subsection{Lower Bounds on The Derived Transport Load}\label{lower-bound-G}

\subsection{Proof of Theorem \ref{Z-D-thm-traffic-load-on-sessions}}
\begin{proof}	
	We present a logical framework for the proof. For conciseness, we refer to several common conclusions from \cite{mobihoc2014, wang2016modeling}. Although the scenario they studied, i.e., online social networks, is indeed a special case for this work, there are still some commonalities in technical logic.
	
	% When the underlying network is involved, the problem of obtaining the optimal transport distance can be reduced to the Euclidean Steiner Tree Problem spanning the set $\{u_k\}\cup\mathbb{D}_k$, where $\mathbb{D}_k$ is the set of all destinations of $u_k$. In this problem, given $|\{u_k\}\cup\mathbb{D}_k|$ nodes in the plane, the objective is to connect them by lines of minimum total length in a way that any two nodes may be interconnected by line segments either directly or via other nodes and line segments \cite{gilbert1968steiner}.
	In the context of the underlying network, the problem of achieving optimal transmission distance involves connecting the nodes in the given plane, which constitutes the set $|{u_k}\cup\mathbb{D}_k|$, where $\mathbb{D}_k$ represents all destinations of $u_k$. % We can use the total length of the Euclidean spanning tree of a session, to measure the order of the total length of the optimal transport distance.
	We can employ the total length of the Euclidean spanning tree of a session to gauge the magnitude of the optimal transport distance.
	This problem can be simplified as generating the Euclidean Steiner tree for the set ${u_k}\cup\mathbb{D}_k$ \cite{gilbert1968steiner}.
	%	The bound on the traffic load depends on the lower bounds on $ \sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}^\mathrm{I}_k)| $.
	%
	%
	% For $k=1,2,\cdots,n_{\mathbb{S}}$, 
	Then, we can get that
	\begin{equation*}
		\begin{aligned}
			%					\widetilde{\mathbf{L}}_{\mathbb{N},\mathcal{S}}(\mathbb{D}_{\mathcal{S}, k})=\lambda\cdot\Omega(|\EMST(\{u_{\mathcal{S},k}\}\cup \mathbb{D}_{\mathcal{S}, k})|), \\
			\mathrm{L}_{\mathrm{N}}^{\ast}= \lambda \cdot\Omega\left( \sum_{k=1}^{n}|\EMST(\{u_{k}\}\cup \mathbb{D}_{k})|\right),
		\end{aligned}
	\end{equation*}
	where $\EMST(\cdot)$ denotes the Euclidean minimum spanning tree \cite{penrose1999strong}.
	
	Further, %we determine the nearest nodes for specific nodes.
	let $\mathcal{A}_k=\{p_{k_1},p_{k_2},\cdots,p_{k_{q_{k}}}\}$ and $\mathcal{F}_k=\{v_{k_1},v_{k_2},\cdots,v_{k_{q_{k}}}\}$ respectively denote the set of  $q_k$ nodes and	the closest nodes to  $p_{k_i}$, for $1 \leq i \leq q_k$.
	%Please see the illustration in Fig.\ref{fig-social-formation}.
	Additionally, we denote a set
	$\mathcal{P}_k= \{v_k\} \cup \mathcal{A}_k$, where $v_k$ is the source from a given session $\mathrm{T}_k$ and call the anchor point of $v_{k_i}$ as $p_{k_i}$.
	Then, for a data transportation session $\mathrm{T}_k$, we can get 
	
	\vspace{-0.11in}
	
	{\small
		\begin{equation*}
			|\EMST(\mathcal{A}_k)|=\Theta(L_{\mathcal{P}}(\mathcal{s}, r_k)), 
			%	\end{equation*}
		%	\begin{equation*}
			|\EMST(\mathcal{P}_{k})|=\Omega(L_{\mathcal{P}}(\mathcal{s}, r_k)),
		\end{equation*}
	}
	
	\vspace{-0.02in}
	
	\noindent where $L_{\mathcal{P}}(\mathcal{s}, r_k)=\sqrt{r_k}\cdot \int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX$. 
	%$\mathbf{d}(Y)=n/m\sum\nolimits_{c_j\in \mathcal{C}} g(Y)/\int_{\mathcal{O}}g(Z)dZ$ 
	%$\mathbf{d}(Y)=\frac{n}{m}\sum\nolimits_{c_j\in \mathcal{C}} \frac{g(Y)}{\int_{\mathcal{O}}g(Z)dZ}$ and $\mathcal{C}$ is the set of points' positions.
	
%	(1) When $ \mathcal{s}>1 $,
%	\begin{equation*}
%		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right)
%	\end{equation*}
%	\begin{equation*}
%		%\Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right) 
%		~~~~~~~~~~~~~~~~~~~~~~=\left\{
%		\begin{array}{ll}
%			\Theta\left(1\right) , & \mathcal{s}>2;\\
%			\Theta\left(\log n\right) , & \mathcal{s}=2;\\
%			\Theta\left(n^{1-\frac{\mathcal{s}}{2}}\right) , & 1<\mathcal{s}<2.
%		\end{array}
%		\right.
%	\end{equation*}
%	
%	
%	(2) When $ \mathcal{s}=1 $,
%	\begin{equation*}
%		\begin{aligned}
%			\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX &= \Theta\left(\frac{1}{\sqrt{\log n}}\cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{1}{2}}}\right)\\
%			& = \Theta\left(\sqrt{\frac{n}{\log n}}\right).
%		\end{aligned}
%	\end{equation*}
%	
%	(3) When $ 0 \leq\mathcal{s} <1 $,
%	\begin{equation*}
%		\begin{aligned}
%			\int_{\mathcal{O}}\sqrt{f_{X_0}(X)} dX &=  \Theta\left(n^{\frac{\mathcal{s}-1}{2}} \cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right)\\
%			&= \Theta\left(\sqrt{n}\right).
%		\end{aligned}
%	\end{equation*}
	
	%	when $ 1<\mathcal{s}<2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right) = \Theta\left(n^{1-\frac{\mathcal{s}}{2}}\right) $;
	%	
	%	when $ \mathcal{s}=2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)}\right) $=$ \Theta\left(\log n\right) $;
	%	
	%	when $ \mathcal{s}>2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\mathcal{s}}{2}}}\right) $=$ \Theta\left(1\right) $.
	In Lemma \ref{lem-EMST-B-D}, the result of $L_{\mathcal{P}}(\mathcal{s}, r_k)$ is in Eq.(\ref{eq-L-P-beta-9765}).
	\begin{equation}
		L_{\mathcal{P}}(\mathcal{s}, r_k) = \left\{
		\begin{array}{ll}
			\Theta\left( \sqrt{r_k} \right)  , &  \mathcal{s}>2;  \\
			\Theta\left(\sqrt{r_k} \cdot \log n  \right), &  \mathcal{s}=2;  \\
			\Theta\left(\sqrt{r_k} \cdot n^{1-\frac{\mathcal{s}}{2}} \right)  , & 1< \mathcal{s} < 2;  \\
			\Theta\left(\sqrt{r_k} \cdot \sqrt{\frac{n}{\log n}} \right) , &  \mathcal{s}=1;  \\
			\Theta\left(\sqrt{r_k} \cdot \sqrt{n} \right)  , &  0\leq\mathcal{s} <1.
		\end{array}
		\right.
	\end{equation}
	
	%	Denote the number of nodes with $ l $ destinations as $ T_{l} $, to simplify the proof, we let
	%	\begin{equation*}
		%		T_{l}  =  n\cdot\mathrm{Pr}(q_{k}=l)  = n\cdot{\left(\sum\nolimits_{j=1}^{n-1}j^{-\mathcal{d}}\right)^{-1}} \cdot l^{-\mathcal{d}}.
		%	\end{equation*}
	%According to Kolmogorov's Strong laws of larger numbers (LLN) \cite{williams1991probability}, it has no impact on the analysis process of issue in order sense. 
	\par First, we consider the \textit{node influence distribution} and we define two sets for all data transportation sessions, where $\mathcal{K}^{1}$ represents the nodes with a constant level of influence $\Theta(1)$, and $\mathcal{K}^{\infty}$ denotes the nodes with a non-constant level of influence. Together, they fully characterize $\sum\nolimits_{k=1}^{n}|\EMST(\mathcal{P}_k)|$. In this proof, ${\Psi}^{1}$ is defined to represent the sum of the lengths of all the Euclidean minimum spanning trees under the condition $k \in \mathcal{K}^{1}$, where ${\Psi}^{1}=\sum_{k \in \mathcal{K}^{1}}|\EMST(\mathcal{P}_k)|$, and ${\Psi}^{\infty}$ is defined to represent the one under the condition $k \in \mathcal{K}^{\infty}$, where ${\Psi}^{\infty}=\sum_{k \in \mathcal{K}^{\infty}}|\EMST(\mathcal{P}_k)|$.
	
	
	%	\begin{equation*}
		%		\mathcal{K}^{1}:=\{k|q_{k}=\Theta(1)\}, \mathcal{K}^{\infty}:=\{k|q_{k}=\omega(1)\}.
		%	\end{equation*}
	%	Then, it follows that
	%	\begin{equation}\label{Transport-sum}
		%		\sum\nolimits_{k=1}^{n}|\EMST(\mathcal{P}^\mathrm{I}_k)|  = \widehat{{\Sigma}}^{1} + \widehat{{\Sigma}}^{\infty},
		%	\end{equation}
	%	where
	%	\begin{equation*}
		%		\widehat{{\Sigma}}^{1} = \sum_{k\in\mathcal{K}^{1}}|\EMST(\mathcal{P}^\mathrm{I}_k)|,
		%		\widehat{{\Sigma}}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}}|\EMST(\mathcal{P}^\mathrm{I}_k)|.
		%	\end{equation*}
	%	We first address the part of $\widehat{{\Sigma}}^{1}$. Since for $q_{k}=\Theta(1)$, it holds that
	%	\[ |\EMST(\mathcal{P}^\mathrm{I}_k)|=\Theta(|X-v_{k}|). \]
	%	Then we have
	%	$ \widehat{{\Sigma}}^{1}=\sum\nolimits_{k\in\mathcal{K}^{1}}|X-v_{k}|. $
	%	For $ k\in\mathcal{K}^{1} $, we define a sequence of random variables
	%	$ \phi^{1}_{k}:=|X-v_{k}|/\sqrt{n} $,
	%	which have finite meaning as follows:
	%	$ E[\phi^{1}_{k}] = E[|X-v_{k}|]/\sqrt{n},$
	%	where $E[|X-v_{k}|]$ is given in Lemma 5 of \cite{mobihoc2014}.
	%	Then, according to Lemma \ref{lem-growthsteel}, with probability $1$, it holds that
	%	\[ \widehat{{\Sigma}}^{1}=\Theta \left(\sqrt{n}\cdot\sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k}\right),\]
	%	and
	%	\begin{equation*}
		%		\sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k} / |\mathcal{K}^{1}|=\Theta(E\left[|X-v_{k}|/\sqrt{n}\right]),
		%	\end{equation*}
	%	where $ |\mathcal{K}^{1}| $ denotes the cardinality of set $ \mathcal{K}^{1} $.
	%	Therefore,
	%	\[ \sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k} = \Theta\left(|\mathcal{K}^{1}|\cdot E\left[|X-v_{k}|/\sqrt{n}\right]\right).\]
	%	Then, by Lemma \ref{lem-Kolmogorov-slln},
	% While ${\Psi}^{1}$ can be calculated from \cite{mobihoc2014} and the result is $\Theta\left(|\mathcal{K}^{1}| \cdot E[|X-v_{k}|] \right)$.
	%	\begin{equation}\label{Transport-for-k-1}
		%		\widehat{{\Sigma}}^{1}=\Theta\left(|\mathcal{K}^{1}| \cdot E[|X-v_{k}|] \right).
		%	\end{equation}
	
	We first address ${\Psi}^{1}$. Since for $q_k=\Theta(1)$, it holds that 	$|\EMST(\mathcal{P}_{k})|=\Theta(|X-v_k|)$. We define a sequence of random variables $\varepsilon_k:=|X-v_k|/\sqrt{n}$, and $\mathbb{E}[\varepsilon_k]=\mathbb{E}[|X-v_k|]/\sqrt{n}$. The value of $\mathbb{E}[|X-v_k|]$ is given in Lemma 5 of \cite{mobihoc2014}. Therefore, ${\Psi}^{1}=\Theta(\sqrt{n}\sum_{k\in \mathcal{K}^{1}}\varepsilon_k )$. Through Kolmogorov's Strong laws of larger numbers (LLM) \cite{williams1991probability}, with probability1,
	\begin{equation*}
		{\Psi}^{1}=\Theta\left(|\mathcal{K}^{1}| \cdot E[|X-v_{k}|] \right).
	\end{equation*}
	
	
	
	Next, we  utilize the \textit{data destination distribution} to consider ${\Psi}^{\infty} $. All $ |\EMST(\mathcal{P}_k)| $ are independent, where $k \in \mathcal{K}^{\infty}$, due to the introduction of anchor points. Similarly to the node influence distribution, we apply the same approach to distinguish the number of nodes selected by this distribution. Specifically, we denote ${\Psi}_{1}^{\infty}$ and ${\Psi}_{\infty}^{\infty}$ as the sum of lengths of all the Euclidean minimum spanning trees under $r_k=\Theta(1)$ and $r_k=\omega(1)$, respectively.
	% For nodes with neighbours number in $ \mathcal{K}^{\infty} $, we define two sets by considering the \textit{content attraction distribution}:
	%	\begin{equation*}
		%		\mathcal{K}^{\infty}_{1} = \{k|d_{k} = \Theta\left(1\right)\}, \mathcal{K}^{\infty}_{\infty} = \{d_{k} = \omega\left(1\right)\}.
		%	\end{equation*}
	%	Then, it follows that
	%	\begin{equation}\label{Transport-for-k-wuqiong}
		%		\widehat{{\Sigma}}^{\infty} =  \widehat{{\Sigma}}_{1}^{\infty} + \widehat{{\Sigma}}_{\infty}^{\infty},
		%	\end{equation}
	%	where
	%	\begin{equation*}
		%		\widehat{{\Sigma}}_{1}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}_{1}}|\EMST \left(\mathcal{P}^\mathrm{I}_k\right)|,
		%		\widehat{{\Sigma}}_{\infty}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}_{\infty}}| \EMST \left(\mathcal{P}^\mathrm{I}_k\right)|.
		%	\end{equation*}
	
	
	%	For $ r_{k} = \Theta\left(1\right) $, the order of $ {\Psi}_{1}^{\infty} $ is lower than that of ${\Psi}^{1} $. For the final summation, the specific value of $ {\Psi}_{1}^{\infty} $ is relatively infinitesimal.
	For $r_k=\Theta\left(1\right)$, the value of $ {\Psi}_{1}^{\infty} $ is relatively infinitesimal compared with ${\Psi}^{1} $.
	
	Then we consider $ \mathcal{K}^{\infty}_{\infty} $. We define $T_q=n\cdot \Pr(q_k=q)=n\cdot \left(\sum_{j=1}^{n-1} j^{-\mathcal{i}}\right)^{-1}\cdot q^{-\mathcal{i}}$, as the number of nodes with $q$ destinations.
	%	With probability $1$, it holds \cite{mobihoc2014} that
	%	\begin{equation*}
		%		|\mathrm{EMST\left(\mathcal{P}^\mathrm{I}_k\right)}| = \Omega\left(L^\mathrm{I}_{\mathcal{P}}(\mathcal{s}, d_k)\right),
		%	\end{equation*}
	%	where $L^\mathrm{I}_{\mathcal{P}}(\mathcal{s}, d_k)$ is defined in Eq.(\ref{eq-L-P-beta-9765}). 
	%		\begin{equation}\label{eq-L-P-beta-9765}
		%				L^\mathrm{I}_{\mathcal{P}}(\mathcal{s}, d_k) = \left\{
		%				\begin{array}{ll}
			%						\Theta\left( \sqrt{d_k} \right)  , &  \mathcal{s}>2;  \\
			%						\Theta\left(\sqrt{d_k} \cdot \log n  \right), &  \mathcal{s}=2;  \\
			%						\Theta\left(\sqrt{d_k} \cdot n^{1-\frac{\mathcal{s}}{2}} \right)  , & 1< \mathcal{s} < 2;  \\
			%						\Theta\left(\sqrt{d_k} \cdot \sqrt{\frac{n}{\log n}} \right) , &  \mathcal{s}=1;  \\
			%						\Theta\left(\sqrt{d_k} \cdot \sqrt{n} \right)  , &  0\leq\mathcal{s} <1.
			%					\end{array}
		%				\right.
		%			\end{equation}
	Through LLN \cite{williams1991probability}, with probability $1$, it holds that
	\begin{equation*}\label{Transport-for-d-wuqiong}
		{\Psi}_{\infty}^{\infty} \geq \sum_{q=2}^{n-1} \sum_{r=1}^{q} T_{q} \cdot \mathrm{Pr}(r_{k}=r|q_{k}=q) \cdot L_{\mathcal{P}}\left(\mathcal{s},r\right).
	\end{equation*}
	Actually, what we should calculate is $\sum_{q=2}^{n-1}\sum_{r=1}^{q}\Pr(q_k=q)\cdot \Pr(r_k=r|q_k=q)$, denoted as $G(\mathcal{i},\mathcal{d})$, which is illuastrated in Table \ref{tab-G}.
	
	Combining with the above conclusions, we can get the lower bounds on $\sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}_k)|$.
	
	\begin{figure*}[t]
		\centering
		\label{pic-understand}
		\vspace{3pt}
		\begin{minipage}{0.32\linewidth}
			%这个图片路径替换成你的图片路径即可使用
			\subfloat[$0\leq \mathcal{d}<1,\mathcal{s}>2$]{\includegraphics[width=\textwidth]{function1.pdf}}
			% 加入对这列的图片说明
			
		\end{minipage}
		\begin{minipage}{0.32\linewidth}
			\subfloat[$0\leq \mathcal{d}<1,\mathcal{s}=2$]{\includegraphics[width=\textwidth]{function2.pdf}}
		\end{minipage}
		\begin{minipage}{0.32\linewidth}
			\subfloat[$0\leq \mathcal{d}<1,1<\mathcal{s}<2$]{\includegraphics[width=\textwidth]{function3.pdf}}
		\end{minipage}
		\begin{minipage}{0.35\linewidth}
			\vspace{10pt}
			\subfloat[$0\leq \mathcal{d}<1,\mathcal{s}=2$]{\includegraphics[width=\textwidth]{function4.pdf}}
		\end{minipage}
		\hspace{10mm}
		\begin{minipage}{0.35\linewidth}
			\vspace{10pt}
			\subfloat[$0\leq \mathcal{d}<1,0<\mathcal{s}<1$]{\includegraphics[width=\textwidth]{function5.pdf}}
		\end{minipage}
		\caption{The order of low bounds on the derived traffic load, under $\lambda=\Theta(1)$ and $0\le \mathcal{d}<1$.}
		\label{thr}
	\end{figure*}

		\begin{table}[t]
		% \renewcommand{\arraystretch}{1.1}
		\centering
		\caption{The Value of $G(\mathcal{i},\mathcal{d})$}
		\label{tab-G}
		%\begin{tiny}
		\renewcommand\arraystretch{1.2}
	\resizebox{0.4\linewidth}{!}{	\begin{tabular}{|l ||l|}
			\toprule
			$\mathcal{d}$ & $ G\left(\mathcal{i}, \mathcal{d}\right) $\\
			\midrule
			
			$\mathcal{d}>\frac{3}{2}$ &
			$ \Theta(1) $  , $ \mathcal{i}\geq0.$ \\
			\midrule
			$\mathcal{d}=\frac{3}{2}$ &
			$\left\{
			\begin{array}{ll}
				\Theta(1)  , &  \mathcal{i} >1; \\
				%\Theta(n \cdot \log n) , &  \mathcal{i}=1;  \\
				\Theta(\log n)  , &  0\leq\mathcal{i}\leq1.
			\end{array}
			\right. $ \\
			\midrule
			$1<\mathcal{d}<\frac{3}{2}$ &
			$\left\{
			\begin{array}{ll}
				\Theta(1) , &  \mathcal{i}>\frac{5}{2}-\mathcal{d};  \\
				\Theta(\log n) , &  \mathcal{i}=\frac{5}{2}-\mathcal{d}; \\
				\Theta(n^{\frac{5}{2}-\mathcal{i}-\mathcal{d}})  , &  1<\mathcal{i}<\frac{5}{2}-\mathcal{d}; \\
				\Theta(n^{\frac{3}{2}-\mathcal{d}} / \log n) , &  \mathcal{i}=1; \\
				\Theta(n^{\frac{3}{2}-\mathcal{d}})  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\midrule
			$\mathcal{d}=1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(1)  , &  \mathcal{i}\geq\frac{3}{2};\\
				\Theta(n^{\frac{3}{2}-\mathcal{i}}/ \log n) , &  1<\mathcal{i}<\frac{3}{2};  \\
				\Theta(n^{\frac{1}{2}} / (\log n)^2) , &  \mathcal{i}=1;  \\
				\Theta(n^{\frac{1}{2}}/ \log n)  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\midrule
			$0\leq\mathcal{d}<1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(1)  , &  \mathcal{i}>\frac{3}{2}; \\
				\Theta(\log n)  , &  \mathcal{i}=\frac{3}{2}; \\
				\Theta(n^{\frac{3}{2}-\mathcal{i}})  , &  1<\mathcal{i}<\frac{3}{2}; \\
				\Theta(n^{\frac{1}{2}}/\log n) , &  \mathcal{i}=1;  \\
				\Theta(n^{\frac{1}{2}})  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\bottomrule
		\end{tabular}
	}
		%\end{tiny}
	\end{table}
	
	\begin{table}[t]
		% \renewcommand{\arraystretch}{1.1}
		\centering
		\caption{The Number of All Destinations, $W\left(\mathcal{i}, \mathcal{d}\right)$}
		\label{tab-W-gamma-varphi}
		%\begin{tiny}
		\renewcommand\arraystretch{1.2}
		\resizebox{0.4\linewidth}{!}{	\begin{tabular}{|l ||l|}
			\toprule
			$\mathcal{d}$ & $ W\left(\mathcal{i}, \mathcal{d}\right) $\\
			\midrule
			$\mathcal{d}>2$ &
			$ \Theta(n) $  , $ \mathcal{i}\geq0.$ \\
			\hline
			$\mathcal{d}=2$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \mathcal{i} >1; \\
				%\Theta(n \cdot \log n) , &  \mathcal{i}=1;  \\
				\Theta(n \cdot \log n)  , &  0\leq\mathcal{i}\leq1.
			\end{array}
			\right. $ \\
			\midrule
			$1<\mathcal{d}<2$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n) , &  \mathcal{i}>3-\mathcal{d};  \\
				\Theta(n \cdot \log n) , &  \mathcal{i}=3-\mathcal{d}; \\
				\Theta(n^{4-\mathcal{i}-\mathcal{d}})  , &  1<\mathcal{i}<3-\mathcal{d}; \\
				\Theta(n^{3-\mathcal{d}} / \log n) , &  \mathcal{i}=1; \\
				\Theta(n^{3-\mathcal{d}})  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\midrule
			$\mathcal{d}=1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \mathcal{i}\geq2;\\
				\Theta(n^{3-\mathcal{i}}/ \log n) , &  1<\mathcal{i}<2;  \\
				\Theta(n^{2} / (\log n)^2) , &  \mathcal{i}=1;  \\
				\Theta(n^{2}/ \log n)  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\midrule
			$0\leq\mathcal{d}<1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \mathcal{i}>2; \\
				\Theta(n \cdot \log n)  , &  \mathcal{i}=2; \\
				\Theta(n^{3-\mathcal{i}})  , &  1<\mathcal{i}<2; \\
				\Theta(n^{2}/\log n) , &  \mathcal{i}=1;  \\
				\Theta(n^{2})  , &  0\leq\mathcal{i}<1.
			\end{array}
			\right. $ \\
			\bottomrule
		\end{tabular}}
		%\end{tiny}
	\end{table}
	
	Then we calculate $\sum\nolimits_{k=1}^n| \mathrm{EMST}(\mathbb{D}_k) |$. Since
	\begin{equation*}
		\sum_{k=1}^{n} r_{k} = \Theta\left(\sum_{q=1}^{n-1} \sum_{r=1}^{q} T_{q} \cdot \mathrm{Pr}(r_{k}=r|q_{k}=q) \cdot r \right),
	\end{equation*}
	where $T_{q}  =  n\cdot\mathrm{Pr}(q_{k}=q) $. We get the result of $ \sum\nolimits_{k=1}^{n} r_{k}$ as $W\left(\mathcal{i}, \mathcal{d}\right)$, as illustrated in Table \ref{tab-W-gamma-varphi}.
	
	Additionally, for all $u_k\in \mathcal{U}$, 
	\begin{equation*}
		E[| v_{k_{i}} - p_{k_{i}} |] =\Theta\left(\int_0^{\sqrt{n}}x\cdot e^{-\pi x^2}dx\right).
		\end{equation*}
	
	That is,
	\begin{equation*}
E[| v_{k_{i}} - p_{k_{i}} |] = \Theta \left(1\right).
	\end{equation*}
	
	% For all $ v_{k} \in \mathcal{V}$,
	%\begin{equation*}
	%	E[| v_{k_{i}} - p_{k_{i}} |] = \Theta\left( \int_{0}^{\sqrt{n}} x \cdot e^{-\pi \cdot x^{2}}dx \right).
	%\end{equation*}
	% That is, \[ E[| v_{k_{i}} - p_{k_{i}} |] = \Theta \left(1\right). \]
	and LLN, with probability $1$, it holds that
	%it holds that
	%\[\frac{\sum_{i=1}^{d_{k}} |v_{k_{i}}-p_{k_{i}}|}{d_{k}}=\Theta(1),\]
	% i.e.,
	% $ \sum_{i=1}^{d_{k}} |v_{k_{i}}-p_{k_{i}}| = \Theta(d_{k}) $.
	%   Then
	\begin{equation*}\label{Length-Anchor-Friends}
		\sum_{k=1}^{n} \sum_{i=1}^{r_{k}} |v_{k_{i}}-p_{k_{i}}| = \Theta\left(\sum_{k=1}^n r_k\right)= \Theta\left(W\left(\mathcal{i}, \mathcal{d}\right)\right).
	\end{equation*}
	Combining the result of $\sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}_k)|$
	%, for all network sessions $\mathbb{D}_k$, $ k = 1, 2, ..., n $, with high probability, it holds that
	%\[ \sum\nolimits_{k=1}^n| \mathrm{EMST}(\mathbb{D}_k) | = \Omega \left(G\left(\mathcal{i}, \mathcal{s}, \mathcal{d}, n\right)\right) .
	% \]
	% of our technical report \cite{dropboxmobihoc2016}.
	and the data arrival rate $\lambda$, we complete the proof.$\hfill\square$
	
	%  of Theorem \ref{Z-D-thm-traffic-load-on-sessions}.
\end{proof}



\subsection{How to Understand Our Results}
%\begin{figure*}[htbp]
%	\centering
%	\begin{minipage}[t]{0.2\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{function1.eps}
%		\caption{World Map}
%	\end{minipage}
%	\begin{minipage}[t]{0.2\textwidth}
%		\centering
%		\includegraphics[width=0.5\textwidth]{function2.eps}
%		\caption{Concrete and Constructions}
%	\end{minipage}
%	\begin{minipage}[t]{0.2\textwidth}
%	\centering
%	\includegraphics[width=0.5\textwidth]{function3.eps}
%	\caption{World Map}
%\end{minipage}
%	\begin{minipage}[t]{0.2\textwidth}
%	\centering
%	\includegraphics[width=0.5\textwidth]{function4.eps}
%	\caption{World Map}
%\end{minipage}
%	\begin{minipage}[t]{0.2\textwidth}
%	\centering
%	\includegraphics[width=0.5\textwidth]{function5.eps}
%	\caption{World Map}
%\end{minipage}
%\end{figure*}

%Our results are based on the interpretation of multiple distributions, as depicted in the Fig. \ref{pic-understand}.  We have discovered that the theoretical representation of traffic load exhibits discontinuities under varying conditions, indicating the potential for significant shifts in real-world scenarios, akin to "phase transitions."  This phenomenon bears resemblance to various adaptations of Metcalfe's Law, where different variants may account for diverse breakpoints and transitions.  This substantiates our belief that our work offers an explanation of Metcalfe's Law from the perspective of traffic load.  Considering our study, further research should explore the rationale behind these breakpoints to validate the variations in traffic load.

%Our conclusions are framed around the interpretation of several delineated distributions, as illustrated in Fig. \ref{pic-understand}. We've observed that the theoretical representation of traffic load displays breakpoints regardless of the conditions, suggesting potential abrupt shifts or ``phase changes" in real-world scenarios due to changing conditions. This phenomenon resonates with the existence of various versions of Metcalfe's Law, where distinct variations may account for diverse breakpoints and transitions. This is why we believe our work provides an interpretation of Metcalfe's Law from the perspective of traffic load. In light of this study, further investigation is warranted to examine the rationale behind these breakpoints, validating the shifts in traffic load under varying conditions.

% Our deductions are centered on the interpretation derived from multiple distributions
Our results are conditioned on multiple distribution indices, represented in Fig. \ref{pic-understand}. We have come to observe that the theoretical depiction of traffic load manifests breakpoints regardless of the conditions, signifying potential ``phase transitions" in real-world scenarios due to varying conditions. These breakpoints play a pivotal role in delineating distinct shifts or transformations within the network dynamics. This observation parallels the existence of multiple variants of Metcalfe's Law, suggesting the presence of diverse breakpoints and transitions, thereby underlining the crucial role these breakpoints hold. This substantiates our belief that our exploration provides a unique perspective on understanding Metcalfe's Law through the lens of traffic load. Building upon this investigation, there's significant value in exploring and validating the impact and significance of these breakpoints in further studies on traffic load dynamics.



==> case.tex <==
%In this section, we provide an explanation of the Metcalfe's Law and its typical variants. Building upon the obtained theoretical results, We establish correspondences between these different families of laws, identifying theoretical conditions and realistic scenarios under which they hold. % Hence, this work aims to demonstrate why Metcalfe's Law is often considered comparable to Moore's Law.
%
%By delving into the intricacies of the various Metcalfe's Law and their related counterparts, the paper offers a comprehensive understanding of their underlying principles. We leverage their theoretical findings to establish connections and draw parallels between these laws, elucidating the factors that contribute to their emergence and applicability.
%In this section, we provide an explanation of Metcalfe's Law and its typical variants. Building upon the obtained theoretical results, we establish correspondences between these different families of laws, identifying theoretical conditions and realistic scenarios under which they hold. By delving into the intricacies of the various Metcalfe's Law and their related counterparts, the paper offers a comprehensive understanding of their underlying principles. We leverage their theoretical findings to establish connections and draw parallels between these laws, elucidating the factors that contribute to their emergence and applicability.

%In this section, we offer an in-depth explanation of Metcalfe's Law and its common variants. Based on our theoretical findings, we establish connections between these different families of laws, identifying the theoretical conditions and real-world scenarios in which they are applicable. By delving into the intricacies of these laws, we gain a comprehensive understanding of their underlying principles. Leveraging our theoretical insights, we draw parallels and establish correspondences between these laws, shedding light on the factors that contribute to their emergence and relevance in various network contexts.
In this section, we offer an in-depth explanation of Metcalfe's Law and its variants. Based on our theoretical findings, we establish connections between these different families of laws, identifying some theoretical exemplary cases and real-world scenarios in which they are applicable. 

%\textbf{Analysis on $\lambda$.}
%In practical applications, the process of data arrival or generation can be influenced by a multitude of factors, including the location of nodes, network infrastructure, user behavior, system capacity, network congestion, user preferences, and technological limitations.
%
%Therefore, we explore the following scenarios: as the number of nodes in a network increases, the data arrival rate $\lambda$ also experiences a corresponding increase, as each node contributes to content production. Consequently, we assume that $\lambda$ is a non-decreasing function of $n$. For the purpose of our analysis in this paper, we consider different scaling behaviors for $\lambda$, specifically $\Theta(1)$, $\Theta(n^{1/2})$, and $\Theta(n)$. These carefully chosen options allow us to examine the influence of varying data arrival rates on the network dynamics and extract meaningful insights.
%Therefore, we consider the following scenarios: as the number of nodes in a network increases, there is a corresponding increase in the data arrival rate $\lambda$ due to each node producing content. Hence, we assume that $\lambda$ is a non-decreasing function of $n$. For the purpose of analysis in this paper, we consider different scaling behaviors for $\lambda$, specifically $\Theta(1)$, $\Theta(n^{1/2})$, and $\Theta(n)$. These choices allow us to investigate the impact of varying data arrival rates on the network dynamics and derive meaningful insights.
%~\\\\
%\par \textbf{Overall Introduction.}
%Based on our theoretical findings, we have matched different laws with their respective conditions, as shown in the Table \ref{tab-law-condition}. In the subsequent sections of this chapter, we will utilize these conditions to explain the real-world implications of these laws, providing theoretical insights into Metcalfe's Law and its variants. To illustrate the significance of Metcalfe's Law, we consider the conditions of several other laws corresponding to different parameter settings, while keeping $\lambda=\Theta(1)$ and $\mathcal{g}=0$, as shown in Fig. \ref{fig:condition}. The range of conditions for each law is depicted in the accompanying graph. It can be observed that the conditions associated with Metcalfe's Law are concentrated within a specific range, yet the occupied area is substantial. From the explanations provided below, we can ascertain that these conditions align well with real-world scenarios. This further demonstrates why Metcalfe's Law holds such a prominent position in the context of network effects.
Here, we provide a concise introduction to the theoretical and physical explanations of the Metcalfe's Law family. Considering the influence of increasing the number of network nodes on the data arrival rate $\lambda$, we assume that $\lambda$ is a non-decreasing function of $n$. In our analysis, we explore different scaling behaviors for $\lambda$, specifically $\Theta(1)$, $\Theta(n^{1/2})$, and $\Theta(n)$. Based on our theoretical findings, we match different laws with their respective exemplary possible cases, as shown in Table \ref{tab-law-condition}. We use these cases to explain the real-world implications of these laws and provide theoretical insights into Metcalfe's Law and its variants. Actually, from Table \ref{tab-W-gamma-varphi}, we can also derive other laws corresponding to different cases. To demonstrate the importance of Metcalfe's Law, we consider the conditions of several other laws corresponding to different parameter settings while keeping $\lambda=\Theta(1)$ and $\mathcal{g}=0$, as shown in Figure \ref{fig:condition}. We provide the explanations for the theoretical conditions and real-world scenarios of Metcalfe's Law and its variants, establishing a bridge between theory and reality. Our proposed four distributions offers theoretical interpretations not only for each law but also for the corresponding scenarios governed by these laws.
%Notably, the conditions associated with Metcalfe's Law are concentrated within a specific range. The explanations provided below confirm that these conditions align well with real-world scenarios, further reinforcing Metcalfe's Law's prominent position in the context of network effects.



\subsection{Original Metcalfe's Law: $n^2$}
%We have summarized and associated the conditions with Metcalfe's Law. Upon examining the table \ref{tab-law-condition}, we can identify the conditions that fulfill the requirements of Metcalfe's Law. Notably, when $\lambda=\Theta(1)$, we observe a consistent alignment with Metcalfe's Law when $\mathcal{s}\geq 0$, $0\leq\mathcal{d}<1$, and $0\leq \mathcal{i}<1$. We observed that when $\mathcal{s}\geq0$, indicating a positive value for the exponent parameter,   Metcalfe's Law held across different ranges of the network. Additionally, we found that for $\mathcal{d}$ and $\mathcal{i}$ values within the interval of $[0, 1)$, which implies a high level of network monopoly and activity, Metcalfe's Law remained applicable. This suggested that as long as the network had a large number of nodes and active users, Metcalfe's Law was suitable for describing its growth and value creation. One prominent example that aligned with these conditions was Online Social Networks (OSNs). In particular, we focused our examination on Facebook and Tencent, two significant social network companies renowned for their extensive user bases and high levels of user activity. The substantial population of users and the active engagement observed within these networks provided strong validation for the applicability of Metcalfe's Law in the context of OSNs, as extensively discussed in the study.
%
%Furthermore, in the case of $\lambda=\Theta(n^{1/2})$, we find five distinct scenarios that yield the same conclusions. When the value of $\mathcal{s}$ fell within $[0,1)$, we inferred that the network was not highly localized and had a more open structure. In this scenario, the larger user base had a significant impact on the rate of data arrival, allowing each node to receive more data per unit of time. However, due to the relatively low level of user activity, we suggested that the exponent parameter, $\lambda$, was likely on the same order of magnitude as $n^{1/2}$, where $n$ represents the number of nodes. Despite this adjustment, our result concludes that this state still conformed to Metcalfe's Law.
%
%In a research conducted by Zhang et al. \cite{zhang2015tencent}, the authors aimed to empirically validate Metcalfe's Law using data obtained from Facebook and Tencent. The dataset encompassed multiple years, offering a comprehensive perspective on the growth and transformation of these networks. Facebook and Tencent are renowned social network companies that have amassed large user bases in their respective regions. As the Internet has advanced, their influence has expanded globally. These companies' extensive operational experience has also fostered a high degree of user engagement. Therefore, Facebook and Tencent serve as prime examples of typical social network entities that align with the conditions we have outlined. Through their meticulous analysis, it was revealed that Metcalfe's Law demonstrated a robust fit across various regions within the dataset, reinforcing its validity and applicability.
%
%Drawing from the results pertaining to traffic load of networks, our conclusion emphasizes the broad applicability of Metcalfe's Law. The law demonstrates validity across diverse parameter spaces, underscoring its relevance and effectiveness in capturing the dynamics of network growth. This extensive applicability has played a pivotal role in establishing the esteemed reputation of Metcalfe's Law since its inception and is evident in the successful verification of its principles using realistic data in the study conducted by Zhang et al. \cite{zhang2015tencent}.
\subsubsection{Theoretical Cases of Metcalfe's Law}
We summarize some possible cases associated with Metcalfe's Law and examined them in Table \ref{tab-law-condition}. It illustrates the scenarios where Metcalfe's Law holds under different values of $\lambda$. Notably, when $\lambda=\Theta(1)$, we observe the consistent alignment with Metcalfe's Law for $\mathcal{s}\geq 0$, $0\leq\mathcal{d}<1$, and $0\leq \mathcal{i}<1$. This suggests that as long as the network has a positive exponent parameter $\mathcal{s}$ and a significant number of active users, Metcalfe's Law is applicable to describe its growth and value creation. A typical example is online social networks, such as Facebook and Tencent, which have extensive user bases and high user engagement.

Additionally, we explore the case of $\lambda=\Theta(n^{1/2})$ and indicate five distinct scenarios yielding similar conclusions. For $\mathcal{s}$ within $[0,1)$, the network is characterized as having a more open structure with a larger node base impacting the rate of data arrival. Our findings indicates that Metcalfe's Law still holds in this state.

\subsubsection{Practical Analysis on Metcalfe's Law}
%To validate the principles of Metcalfe's Law, Zhang et al. \cite{zhang2015tencent} conducted empirical research using data from Facebook and Tencent. The dataset encompassed multiple years, offering a comprehensive perspective on the growth and transformation of these networks. Facebook and Tencent are prime examples of social network entities aligning with the conditions outlined in our study. The analysis reveals that Metcalfe's Law demonstrates a robust fit across various regions within the dataset, reinforcing its validity and applicability.
%
%% Our research underscores the broad applicability of Metcalfe's Law, capturing the dynamics of network growth across diverse parameter spaces.
%Moreover, our research emphasizes the broad applicability of Metcalfe's Law, capturing the dynamics of network growth across diverse parameter spaces. By exploring the growth and transformation of these networks, we gain deeper insights into the underlying principles governing network behavior. The findings highlight the significance of Metcalfe's Law in understanding and predicting the evolution of social networks and other interconnected systems.

To validate the principles of Metcalfe's Law, Zhang et al. \cite{zhang2015tencent} conducted an empirical research study utilizing data from two prominent social network entities, Facebook and Tencent. The dataset covers multiple years, providing a comprehensive perspective on the growth and transformation of their networks. Both Facebook and Tencent exemplify social networks that match the conditions outline in our study. The analysis of the data reveals that Metcalfe's Law consistently demonstrates a robust fit across various regions within the dataset, thereby reinforcing its validity and applicability.

Through our research, we emphasize the wide-ranging applicability of Metcalfe's Law, as it effectively captures network growth across diverse parameter spaces. The study showcases how the law's underlying principles hold in the context of various social networks, serving as a valuable tool for understanding and predicting network behavior and value.

\begin{table}[t] \renewcommand{\arraystretch}{1.5}
	
	\caption{Some Exemplary Possible Cases of \\ the Representative Scaling Laws}
	\label{tab-law-condition} \centering
	
	\resizebox{0.7\linewidth}{!}{	   
		\begin{tabular}{|l|l|}
			\toprule Representative Scaling Laws& Some Exemplary Possible Cases
			\\
			\midrule
			%$\mu_{\mathrm{s}} \in [0,1] $         &  scaling exponent of deployment region
			%\\
			%\hline
			%$\mu_{\mathrm{c}} \in [0,1] $ &   density exponent of centers
			%\\
			%\hline
			\multirow{6}{*}{Metcalfe's Law: $n^2$} 
			& $\lambda=\Theta(1),\mathcal{s}\geq 0,0\leq\mathcal{d}<1,0\leq \mathcal{i}<1;$
			\\
			& $\lambda=\Theta(n^{1/2}),0\leq\mathcal{s}<1,\mathcal{d}>3/2,\mathcal{i}\geq 0;$
			\\
			& $\lambda=\Theta(n^{1/2}),0\leq \mathcal{s}<1,\mathcal{d}=3/2,\mathcal{i}>1;$
			\\
			& $\lambda=\Theta(n^{1/2}),0\leq \mathcal{s}<1,1<\mathcal{d}<3/2,\mathcal{i}>5/2-\mathcal{d};$
			\\
			& $\lambda=\Theta(n^{1/2}),0\leq \mathcal{s}<1,\mathcal{d}=1,\mathcal{i}\geq 2;$
			\\
			& $\lambda=\Theta(n^{1/2}),0\leq \mathcal{s}<1,0\leq\mathcal{d}<1,\mathcal{i}>3/2.$
			\\
			
			\midrule
			
			\multirow{5}{*}{Sarnoff's Law: $n$} 
			& $\lambda=\Theta(1),\mathcal{s}>2,\mathcal{d}>2,\mathcal{i}\geq0;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,\mathcal{d}=2,\mathcal{i}>1;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,1<\mathcal{d}<2,\mathcal{i}>3-\mathcal{d};$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,\mathcal{d}=1,\mathcal{i}\geq 2;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,0\leq\mathcal{d}<1,\mathcal{i}>2.$
			\\
			\midrule
			
			\multirow{5}{*}{Odlyzko's Law: $n\log n$} 
			& $\lambda=\Theta(1),\mathcal{s}=2,\mathcal{d}\geq2,\mathcal{i}\geq0;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,\mathcal{d}=2,0\leq\mathcal{i}<1;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}=2,1\leq\mathcal{d}<2,\mathcal{i}\geq3-\mathcal{d};$
			\\
			& $\lambda=\Theta(1),\mathcal{s}>2,0\leq\mathcal{d}<1,\mathcal{i}=2;$
			\\
			& $\lambda=\Theta(1),\mathcal{s}=2,0\leq\mathcal{d}<1,\mathcal{i}\geq2.$
			\\
			\midrule
			
			\multirow{1}{*}{Cube Law: $n^3$} 
			& $\lambda=\Theta(n),\mathcal{s}\geq 0,0\leq\mathcal{d}<1,0\leq \mathcal{i}<1.$
			\\
			\bottomrule
		\end{tabular}
		
	}
	% \vspace{-0.3cm}
\end{table}
\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{Condition.eps}
	\caption{The scope of different laws corresponding to the conditions while $\lambda=\Theta(1)$. It can be noticed that the region associated with Metcalfe's Law is the most concentrated. We remark that under the condition $\lambda=\Theta(1)$, the cube law has no corresponding conditions.}
	\label{fig:condition}
	\vspace{-0.5cm}
\end{figure}
\subsection{Sarnoff's Law: $n$}

\subsubsection{Theoretical Cases of Sarnoff's Law}
%The conditions for the validity of Sarnoff's Law include the following cases when $\lambda=\Theta(1)$: $\mathcal{s}>2,\mathcal{d}>2,\mathcal{i}\geq0$; $\mathcal{s}>2,\mathcal{d}=2,\mathcal{i}>1$; $\mathcal{s}>2,1<\mathcal{d}<2,\mathcal{i}>3-\mathcal{d}$; $\mathcal{s}>2,\mathcal{d}=1,\mathcal{i}\geq 2$; and $\mathcal{s}>2,0\leq\mathcal{d}<1,\mathcal{i}>2$. These conditions are characterized by a high degree of localization and a substantial yet limited number of active nodes.
%
%
%When the level of openness within a network is restricted below a certain threshold, the interaction between nodes becomes more constrained, particularly in situations where the activity level of the nodes is relatively low. Therefore, the amount of data transmitted between nodes within a unit of time significantly decreases. Hence, using a constant level of $\lambda$ in such a scenario is justified.
% As a result, the amount of data transmitted between nodes is significantly reduced, thereby justifying the use of a constant level, denoted as $\lambda$, in such scenarios.
The possible cases for Sarnoff's law are illustrated in Table \ref{tab-law-condition}. These scenarios are characterized by strong regional correlations and low-degree distributions.
% include: $\lambda=\Theta(1)$ with specific parameter ranges: $\mathcal{s}>2,\mathcal{d}>2,\mathcal{i}\geq0$; $\mathcal{s}>2,\mathcal{d}=2,\mathcal{i}>1$; $\mathcal{s}>2,1<\mathcal{d}<2,\mathcal{i}>3-\mathcal{d}$; $\mathcal{s}>2,\mathcal{d}=1,\mathcal{i}\geq 2$; and $\mathcal{s}>2,0\leq\mathcal{d}<1,\mathcal{i}>2$. 

In networks characterized by limited openness, interactions between nodes are more constrained, especially when node activity levels are relatively low. Consequently, the amount of data transmitted between nodes within a given time period is significantly reduced. Therefore, it is reasonable to use a constant level of $\lambda$ in such scenarios.

In such networks, the information flows between nodes are hindered due to the restricted nature of node interactions, which may arise from factors such as access permissions of the device. As a result, the level of data transmission within the network remains minimal, with limited exchange of information among nodes.

\subsubsection{Practical Analysis on Sarnoff's Law}
%These conditions primarily apply to networks that exhibit a strong degree of localization and possess a large but restricted number of active users. As a result, there is minimal overlap between nodes within the network. Sarnoff's Law was originally proposed within the context of television networks, which are widely present in households but have limited interactivity, leading to a relatively lower prominence of value derived from user interactions.
%
%
%Sarnoff's Law was originally formulated to describe the dynamics of broadcast media platforms, including television and other similar media channels.  These networks typically operate with limited interaction among users, as the primary function involves the transmission of information from broadcasting nodes to viewers.  As a result, the network's traffic and value are predominantly determined by the number of nodes present in the network.
%
%In broadcast media networks, the value of the network is closely tied to the quantity of nodes, rather than the level of user interaction or engagement.  The main focus is on the dissemination of content from a central source to a large audience, with little to no direct interaction between viewers.  Therefore, the success and value of these networks are primarily measured by the reach and size of their audience.
%
%It is worth noting that the applicability of Sarnoff's Law may be limited to specific types of networks, such as broadcast media platforms, where the emphasis lies on the one-way transmission of content.  In other network models with more interactive and participatory elements, the relationship between the number of nodes and the network's value may differ.

%The conditions for Sarnoff's Law are primarily applicable to networks characterized by strong localization and a large yet restricted number of active users, resulting in minimal overlap between nodes. Originally formulated for broadcast media platforms, such as television and similar media channels, these networks operate with limited interaction among users, as their main function involves transmitting information from broadcasting nodes to viewers. Thus, the network's traffic and value primarily depend on the number of nodes present in the network, and success is measured by the reach and size of the audience.
The conditions for Sarnoff's Law primarily apply to networks with strong localization and a large but limited number of active users, leading to minimal node overlap. Originally formulated for broadcast media platforms, such as TV and similar channels, these networks have limited user interaction, focusing on one-way information transmission from broadcasting nodes to viewers. Hence, the network traffic and value depend on the number of nodes linearly.

In broadcast media networks, the value of the network is closely tied to the quantity of nodes, rather than the level of user interaction or engagement.  The main focus is on the dissemination of content from a central source to a large audience, with little to no direct interaction between viewers.  Therefore, the value of these networks are primarily measured by the reach and size of their audience.


\subsection{Odlyzko's Law: $n\log n$}
\subsubsection{Theoretical Cases of Odlyzko's Law}
For Odlyzko's Law, we have identified several exemplary cases under the assumption demonstrated in Table \ref{tab-law-condition}. These conditions indicate a high level of relationship under a  limited region, a large number of potential nodes, and relatively fewer destinations for nodes to select.

This set of conditions is associated with networks that exhibit strong localization, where the majority of nodes have limited connections and there are fewer active nodes. In such networks, the value of the network primarily stems from the potential user base rather than active user engagement. Odlyzko's Law challenges Metcalfe's Law by emphasizing that the value growth of communication networks is not solely dependent on the number of active connections but also considers the potential reach of the network.

Note that the applicability of Odlyzko's Law is contingent upon the specific conditions outlined above. These conditions highlight the characteristics of networks where the value growth is primarily driven by the potential user base rather than the level of active engagement.

\subsubsection{Practical Analysis on Odlyzko's Law}
One typical example is carrier networks \cite{briscoe2006metcalfe}. In the carrier networks, it is a common practice for large ISPs (Internet Service Providers) to decline peering arrangements with smaller operators. These networks demonstrate a pronounced localization, a substantial user base potential, and relatively low user activity levels. In this context, the primary emphasis lies on interconnection between operators rather than extensive user-to-user interconnection. Consequently, the overall number of actively participating nodes within the network remains comparatively limited.

Different from the conditions outlined in Sarnoff's Law, networks guided by Odlyzko's Law exhibit a slightly elevated level of interactivity.
% However, interconnection among users is generally low or nearly absent. Consequently, the network's overall architecture is primarily focused on interconnection between operators rather than direct user-to-user interaction. 
In general, user-to-user interconnection within the network is limited or almost non-existent. As a result, the network's predominant architecture centers around facilitating interconnection between operators rather than facilitating direct interactions between users.
In such a context, the number of actively engaged nodes remains constrained.

When taking into account these attributes, it is reasonable to introduce a factor of $\log n$, to capture the slightly heightened interactivity relative to Sarnoff's Law. This factor acknowledges the logarithmic growth in network effects stemming from the constrained interconnection among users within these networks \cite{briscoe2006metcalfe}.

% In summary, the networks corresponding to Odlyzko's Law demonstrate a notable localization, a substantial user base, and constrained user-to-user interconnection.  Although relatively more interactive compared to Sarnoff's Law situations, the total count of active nodes remains limited, necessitating the inclusion of a logarithmic factor to appropriately capture the network effects.

%One typical example is carrier networks \cite{briscoe2006metcalfe}. In carrier networks, large ISPs often decline peering arrangements with smaller operators, leading to pronounced localization, a substantial user base potential, and relatively low user activity levels. The primary emphasis lies in interconnection between operators rather than extensive user-to-user interconnection, resulting in a comparatively limited number of actively participating nodes.
%
%Odlyzko's Law depicts networks with slightly elevated interactivity, but low or nearly absent interconnection among users. The network's architecture is primarily focused on interconnection between operators, leading to constrained direct user-to-user interaction. To appropriately capture the network effects in such contexts, a factor of $\log n$ is introduced, acknowledging the logarithmic growth stemming from constrained user interconnection \cite{briscoe2006metcalfe}.




\subsection{Cube Law: $n^3$}
%As the number of users increases, the amount of incoming information per unit of time may approach the magnitude of the total user count, as evidenced by data from 2020 \cite{zhang2023facebook} that aligns more closely with an order of $n^3$.
\subsubsection{Theoretical Cases of Cube Law}
As the number of users increases, the amount of incoming information within a unit of time may approach the total number of users, as demonstrated by the data from Zhang et al. \cite{zhang2023facebook} in 2020. The conditions are shown in Table \ref{tab-law-condition}, while we select $\lambda=\Theta(n)$.

This trend emphasizes the importance of considering the growing user count when analyzing the information flow in networks. With an expanding user base, the network becomes more vibrant, fostering increased interactions and information sharing among users. The continuous growth in user numbers amplifies the rate of information arrivals, underscoring the notion that user interactions become increasingly intertwined as the user base expands.

\subsubsection{Practical Analysis on Cube Law}
%Several factors contribute to this observation. Firstly, a larger user base results in a larger pool of active participants in the network. With more active users generating and sharing information, the overall rate of information arrivals naturally increases. Additionally, the expanding user base brings a wider range of interests and content being shared within the network. This diversity stimulates more interactions among users, leading to a higher rate of information arrivals.
%
%The study by Zhang et al. \cite{zhang2023facebook} highlights the impact of a larger user population, demonstrating intensified interaction and engagement among users. The rate of information arrivals closely approximates the magnitude of the total user count, indicating a highly interconnected network where users actively exchange information.

%Several factors contribute to this observation. Firstly, a larger user base results in a larger pool of active participants in the network. With more active users generating and sharing information, the overall rate of information arrivals naturally increases. Additionally, the expanding user base brings a wider range of interests and content being shared within the network. This diversity stimulates more interactions among users, leading to a higher rate of information arrivals.
%
%Furthermore, as the number of nodes increases, we can observe that the relationship between network value and network traffic surpasses a linear correlation. Analyzing real-world scenarios, this observation appears to be reasonable. For example, in online social networks, each new user brings with them additional content, connections, and interactions, thereby enhancing the overall user experience and attracting more users to join. Furthermore, economies of scale may come into play, where the network's infrastructure and resources become more efficient and cost-effective as the number of users increases. Consequently, in \cite{zhang2023facebook}, the exploration of social network data up to the year 2020 reveals a better fit with the cube law, indicating a highly interconnected network where users actively exchange information. This suggests that a larger user base brings greater economies of scale.


There are several factors that contribute to the observed phenomenon. Firstly, a larger user base in the network leads to a higher number of active participants. As more users engage in generating and sharing information, the overall rate of information arrivals naturally increases. This influx of data contributes to a dynamic and vibrant network ecosystem.

%Moreover, the expanding user base brings with it a diverse array of interests and content being shared within the network. This diversity fosters more interactions among users, creating a network that is rich in connections and communication. As a result, the rate of information arrivals continues to rise, fueled by the interactions and exchanges between users.





Additionally, with the increase in the number of nodes in the network, we observe a shift in the relationship between network value and network traffic. The traditional linear correlation is surpassed as the network scales. Real-world scenarios, particularly evident in online social networks, exemplify this trend. Each new user joining the network brings a wealth of additional content, connections, and interactions, all contributing to an enhanced user experience. This positive user experience attracts even more users to join the network, resulting in a self-reinforcing cycle of growth.


\begin{figure}[t]
	\centering
	\includegraphics[width=0.48\textwidth]{final-map.pdf}
	\caption{The user distribution map of Gowalla illustrates the geographical spread plotted against latitude and longitude. Utilizing this information, we pinpointed two specific areas for closer examination in Fig. \ref{fig_gowalla} to assess the rationale behind setting $\mathcal{g}=0$ in this study.}
	\label{fig:final_map}
	\vspace{-0.5cm}
\end{figure}
\begin{figure}[t]
	\centering
	% \label{pic-understand}
	%\vspace{3pt}
	\begin{minipage}{\linewidth}
		%这个图片路径替换成你的图片路径即可使用
		\subfloat[Bloomington in Illinois]{\includegraphics[width=\textwidth]{Gowalla1.pdf}}
		% 加入对这列的图片说明
		
	\end{minipage}
	\begin{minipage}{\linewidth}
		\subfloat[San Francisco in California]{\includegraphics[width=\textwidth]{Gowalla2.pdf}}
	\end{minipage}
	\vspace{-0.1in}
	\caption{The geographical position of Gowalla Users in Illinois and California, respectively.}
	\label{fig_gowalla}
\end{figure}

Furthermore, economies of scale play a significant role in this phenomenon. As the number of users increases, the network's infrastructure and resources become more efficient and cost-effective. This, in turn, enables the network to handle higher traffic loads and accommodates the growing user base without compromising on performance.

A compelling example of these observations is evident in \cite{zhang2023facebook}, where the analysis of social network data up to the year 2020 reveals a better fit with the cube law. The cube law suggests a highly interconnected network, where users actively exchange information and contribute to the overall network value. This further reinforces the notion that a larger user base brings about greater economies of scale, driving network growth and efficiency.


==> conclusion.tex <==
%In this study, our focus revolves around Metcalfe's Law and its variants as we aim to provide a theoretical perspective on network value, specifically in relation to network traffic load.% To enhance the subsequent interpretation of the existing law, we expand the number of parameters based on previous studies such as \cite{mobihoc2014, wang2016modeling}, offering more possibilities for analysis.
%
%We strive to establish connections between the existing Metcalfe's Law and its variants by aligning them with theoretical conditions and considering realistic scenarios. This approach enables us to provide reasonable interpretations for the data validation work that has been conducted thus far.
%
%Moving forward, future research could delve into a more in-depth theoretical analysis of the parameters involved, ultimately leading to a more comprehensive interpretation of the scenarios governed by Metcalfe's Law. By further exploring the intricacies of these parameters, we can gain a deeper understanding of the underlying mechanisms driving network value creation.
%
%In summary, our work aims to provide a theoretical framework for understanding network value based on Metcalfe's Law and its variants, with a specific focus on network traffic load. Expanding the parameters and considering realistic scenarios allows us to offer meaningful interpretations of the existing data validation efforts. Subsequent studies can build upon these findings, focusing on a more thorough analysis of the parameters to enhance our understanding of Metcalfe's Law in various network contexts.

% 重写conclusion

% This study primarily focuses on providing a theoretical interpretation of Metcalfe's Law, aiming to explain it and its related variants from the perspective of network traffic load.  We begin by summarizing a comprehensive network framework for existing network models, where all nodes can function both as data generators and data receivers.  Within this network framework, we define four layers of parameters to constrain the computation of network traffic load.  After obtaining theoretical results, we offer the explanations for Metcalfe's Law and its variants, bridging some theoretical exemplary possible cases of the laws with real-world scenarios, thereby highlighting the significance of Metcalfe's Law.

% This study mainly focuses on theoretical explanation of Metcalfe's law and its variants. From the perspective of network traffic loadi, this study gives some possible theoretical conditions which Metacalfe's law and its variants hold, and corresponds these laws to realistic scenarios. This theoretically shows that these laws do not appear in the same scenarios and have their own existence. At the same time, we give theoretical results in the complete parameter domain, which can provide theoretical guidance for the study of scenarios corresponding to the discovery of new scalar laws other than the above laws in the future.

% This study primarily focuses on providing a theoretical explanation of Metcalfe's Law and its variants from the perspective of network traffic load. We establish possible theoretical conditions under which Metcalfe's Law and its variants hold and correlate these laws with real-world scenarios. The theoretical analysis reveals that these laws are applicable in distinct scenarios and have their unique significance. Additionally, we present theoretical results across a complete parameter space, offering valuable insights for exploring scenarios associated with the discovery of new scaling laws beyond the ones mentioned above in the future.

This study primarily focuses on providing a theoretical explanation of Metcalfe's Law and its variants from the perspective of network traffic load. To address the limits of these laws, we establish the potential theoretical conditions under which Metcalfe's Law and its variants hold and correlate these laws with real-world scenarios. The theoretical analysis reveals that these laws are applicable in distinct scenarios and have their unique significance. Particularly, we present the theoretical results across the complete parameter space for a general network model, offering valuable insights for exploring scenarios associated with the discovery of new scaling laws beyond the ones mentioned above in the future.
To the best of our knowledge, this is the first theoretical
explanation on Metcalfe’s Law and its variants.

%This study is centered on providing a theoretical interpretation of Metcalfe's Law, with a specific focus on understanding it in relation to network traffic load.   To achieve this, we first establish a comprehensive network framework that encompasses existing network models, allowing all nodes to act both as data generators and data receivers.   Within this framework, we define four layers of parameters that play a crucial role in constraining the computation of network traffic load.
%We gain valuable insights of traffic load.   This exploration leads us to offer explanations for Metcalfe's Law and its variants, unveiling the specific conditions they satisfy under different contexts.   Such elucidation highlights the significance of Metcalfe's Law and contributes to a deeper understanding of its implications in various network scenarios.
%The insights gained from this study offer valuable perspectives for future research and practical applications in the field of network analysis and optimization.

==> discussion.tex <==
To further indicate the connection between our work and the Metcalfe's Law family, this section delves into the universality of the proposed network framework and explores the relationship between the traffic load and value of networks.

% \subsection{Feasibility Analysis of the Network}
%With the rapid advancement of communication technology, the landscape of data transmission over networks has undergone a profound transformation, witnessing a proliferation of diverse data formats and an expansion of the applications utilizing these networks in various aspects of daily life and production.  This evolution has further accentuated the significance and relevance of networks in our modern society.

$\bullet$ In our model, each individual node within the network possesses the capability to not only act as a data receiver but also as a data source. This assumption is supported by empirical evidence in real-life scenarios. Across the spectrum of communication technologies, ranging from the deployment of 4G in mobile internet to the revolutionary implementation of 5G in the Internet of Things (IoT), this dual functionality of network nodes has consistently manifested itself. The introduction of this generic model provides numerous possibilities for information dissemination, collaborative data exchange, and peer-to-peer communication.

%By embracing this practical and unified model of network architecture, we set the stage for a comprehensive exploration of its implications and applications.  The versatility of nodes being able to initiate data transmission or passively receive data brings about a myriad of possibilities in terms of information dissemination, collaborative data exchange, and peer-to-peer communication, and so on.

% By adopting this practical and unified network architecture paradigm, we lay the foundation for comprehensive exploration of its significance and applications. Nodes can engage in both data generation and data reception, providing numerous possibilities for information dissemination, collaborative data exchange, and peer-to-peer communication.

% \subsection{The Relationship between Network Value and Traffic Load}
$\bullet$ In our study, we quantify network value through network traffic load, as both are generated by the demands of network nodes.
In our everyday understanding, a prevailing consensus suggests \textit{traffic is value}. However, the direct equivalence between traffic and value might not be absolute. This is due to the characteristics of data transmission in networks, where the upper limit of network value is somewhat influenced by traffic. Nevertheless, there undoubtedly exists a positive correlation between these two factors.
% The demands of nodes within the network necessitate support from traffic, and meeting these demands contributes to the overall value of the network.
%In our study, we delve into the concept of network value, which we quantify through network traffic load.  The value of a network becomes evident when the diverse needs of nodes within it are effectively fulfilled.  Unlike individual nodes operating in isolation, the fundamental purpose of a network is to cater to these node requirements by facilitating seamless data transmission, ultimately giving rise to the generation of network traffic.  It is within this traffic load that the intrinsic value of the network is manifested.
However, the metric of network value lacks a stringent formalization at present, presenting a challenge in precisely assessing its true worth. To address this, we adopt an assumption of a linear relationship between network value and traffic load, a crucial basis for drawing our conclusions.  Nevertheless, we recognize the necessity to embark on future research endeavors aimed at establishing a rigorous and well-defined measurement standard for network value. We aim to achieve a deeper and more comprehensive understanding of Metcalfe's Law, which dictates the relationship between a network's value and its traffic load.

% 加一段 关于算网的future work
%$\bullet$ In this paper, we investigate a generic network structure where the lower layer represents hardware infrastructure support, while the upper layer handles application connections, transmitting data and information.  Based on data form and content, we have identified four distributions to govern network traffic.  In this chapter, we introduce a novel network paradigm called the Computational Power Network (CPN).  In a CPN, computational resources encompass servers, computers, embedded devices, and other computing equipment.  These devices connect to a shared network, facilitating data exchange and collaboration for intricate computational tasks.  High-speed interconnections are typically employed within CPNs to ensure rapid data transmission and processing.
%
%At an abstract level, what distinguishes the CPN from conventional network structures is its transmission of "models."  In essence, however, the CPN still conveys data and computational instructions, placing it squarely within the framework we've delineated.  Among the four defined distributions, the data destination distribution holds particular relevance for the CPN, as it directly correlates with computational scheduling.  This distribution is of paramount significance, accentuating the unique characteristics of the CPN.

%$\bullet$ Furthermore, we introduce the Computational Power Network (CPN) in this chapter, where computational resources, including servers, computers, embedded devices, and other computing equipment, connect to a shared network. This setup fosters data exchange and collaboration for complex computational tasks, often utilizing high-speed interconnections.
%At an abstract level, what sets CPNs apart from conventional network structures is their transmission of \textit{models}. However, in essence, CPNs still convey data and computational instructions, firmly aligning them with the framework we have outlined. Of the four defined distributions, the data destination distribution is particularly pertinent to CPNs as it directly influences computational scheduling, underscoring the distinctive attributes of the CPN.

==> evaluation.tex <==





In this section, we provide an evaluation of the parameters in the theoretical model by utilizing several relevant datasets.
While prior work has extensively explored data validation of Metcalfe's Law and its variants, these validations have been conducted separately in various network contexts. To verify both Metcalfe's Law and its variants and to assess the validity of our proposed theoretical framework, we divide our experiments into two parts.


%In the first part, we initially validate our original Network Geography Distribution, ensuring its alignment with real-world scenarios. In the second part, we turn our attention to calculating network traffic using datasets for further empirical validation.

In the initial segment, we conduct an initial validation of our Network Geography Distribution, affirming its alignment with real-world scenarios. In the subsequent section, our focus shifts to the computation of network traffic using datasets, providing further empirical validation.

\subsection{Network Geography Distribution}

In this section, we provide the evaluations of the network geography distribution through the Gowalla dataset. The Gowalla dataset is a comprehensive collection of location-based information obtained from the Gowalla social networking platform. It predominantly emphasizes geospatial data associated with check-ins and user activities across diverse physical locations.  Each check-in record generally encompasses details such as geographical coordinates (latitude and longitude) of the location, a timestamp, and occasionally supplementary metadata like the place's name or venue category.
This dataset presents a diverse and extensive assortment of geographic information, facilitating analyses concerning user mobility patterns, location-based recommendations, and insights into human behavior linked with spatial interactions.

In Fig. \ref{fig:final_map}, we present the overall geographical distribution of Gowalla users in the United States, utilizing a Mercator projection coordinate system. Building upon this, we select two specific locations to examine the distribution of geographical positions, as illustrated in Fig. \ref{fig_gowalla}, providing further clarification for the configurations.

% In our evaluaions, we extracted 29,105 and 84,222 users who located in Bloomington in Illinois (85\degree W-92\degree W and 37\degree N-45\degree N) and San Francisco in California (121\degree W-122\degree W and 37\degree N-38\degree N), respectively. Following an analysis of the dataset illustrated in Fig. \ref{fig_gowalla}, we observe that the distribution of geographical positions within real-world networks also tends to exhibit a preference for uniformity. This finding significantly supports the validity of our underlying assumption.

In our evaluations, we specifically extract data from 29,105 users in Bloomington, Illinois (within the coordinates 85\degree W - 92\degree W and 37\degree N - 45\degree N, Fig. \ref{fig_gowalla}(a)), and 84,222 users in San Francisco, California (within the coordinates 121\degree W - 122\degree W and 37\degree N - 38\degree N Fig. \ref{fig_gowalla}(b)). Subsequent to a detailed analysis of the dataset, a noticeable trend emerges: the geographical distribution within real-world networks tends to favor uniformity. This observation robustly supports the credibility of our underlying assumption.


\begin{figure*}[t]
	\centering
	% \vspace{3pt}	
	\subfloat[Sarnoff's Function $y=an+b$]{\begin{minipage}{0.24\linewidth}
			%这个图片路径替换成你的图片路径即可使用
			\includegraphics[width=\textwidth]{01.pdf}
			% 加入对这列的图片说明
		\end{minipage}
		\begin{minipage}{0.24\linewidth}
			\includegraphics[width=\textwidth]{02.pdf}
	\end{minipage}	}
	\subfloat[Odlyzko's Function $y=an\ln n+bn +c$]{\begin{minipage}{0.24\linewidth}
			%这个图片路径替换成你的图片路径即可使用
			\includegraphics[width=\textwidth]{11.pdf}
			% 加入对这列的图片说明
		\end{minipage}
		\begin{minipage}{0.24\linewidth}
			\includegraphics[width=\textwidth]{12.pdf}
	\end{minipage}}
	
	\subfloat[Metcalfe's Function $y=an^2+bn +c$]{\begin{minipage}{0.24\linewidth}
			%这个图片路径替换成你的图片路径即可使用
			\includegraphics[width=\textwidth]{21.pdf}
			% 加入对这列的图片说明
		\end{minipage}
		\begin{minipage}{0.24\linewidth}
			\includegraphics[width=\textwidth]{22.pdf}
	\end{minipage}}
	\subfloat[Cube Function $y=an^3+bn^2 +cn+d$]{\begin{minipage}{0.24\linewidth}
			%这个图片路径替换成你的图片路径即可使用
			\includegraphics[width=\textwidth]{31.pdf}
			% 加入对这列的图片说明
		\end{minipage}
		\begin{minipage}{0.24\linewidth}
			\includegraphics[width=\textwidth]{32.pdf}
	\end{minipage}}
	\caption{The empirical curve fitting results of Metcalfe's law and its variants, which can be seen as $y=an+b,y=an\ln n +bn+c, y=an^2+bn+c, y=an^3+bn^2+cn+d$, corresponding to Sarnoff's function, Odlyzko's function, Metcalfe's function and Cube function, repectively.}
	\label{pic-fit}
	\vspace{-0.1in}
\end{figure*}

\begin{table*}[t] \renewcommand{\arraystretch}{1.2}
	
	\caption{Empirical Result of Metcalfe's Law and its Variants}
	\label{tab-law-fit} \centering
	
	\resizebox{0.9\linewidth}{!}{    
		\begin{tabular}{|l|l|l|l|l|}
			\toprule & Given Day&Number of Nodes $n$ & Interaction Types & Value Function              \\ \midrule
			\multirow{2}{*}{Sarnoff's function}  &3& 110            &Call-out& $\mathrm{L}^*_{\mathrm{N}}(n)=2.34n$                     \\ \cmidrule{2-5}
			&4&150             &Call-out                        & $\mathrm{L}^*_{\mathrm{N}}(n)=4.43n$                     \\ \midrule
			\multirow{2}{*}{Odlyzko's function}  & 4&20         &Call-out     & $\mathrm{L}^*_{\mathrm{N}}(n)=-0.5n\ln n+4.71n-2.99$       \\ \cmidrule{2-5}
			&     6 & 20             & Call-in                  & $\mathrm{L}^*_{\mathrm{N}}(n)=0.48n\ln n+3.02$       \\ \midrule
			\multirow{2}{*}{Metcalfe's function} & 25&80           &Call-out & $\mathrm{L}^*_{\mathrm{N}}(n)=0.094n^2+74.65$            \\ \cmidrule{2-5}
			&  25   & 160                & SMS-out             & $\mathrm{L}^*_{\mathrm{N}}(n)=0.034n^2+101.14$            \\ \midrule
			\multirow{2}{*}{Cube function}       &12& 60                &Call-in& $\mathrm{L}^*_{\mathrm{N}}(n)=0.0021n^3-0.129n^2+5.82n$  \\ \cmidrule{2-5}
			&     8  &       80                      &SMS-out& $\mathrm{L}^*_{\mathrm{N}}(n)=0.0011n^3-0.088n^2+5.25n$ \\ \bottomrule
		\end{tabular}
		
	}
	\vspace{-0.3cm}
\end{table*}


\subsection{Traffic Load}
We use the Milan dataset \cite{barlacchi2015multi} for traffic evaluation. The Milan dataset comprises Internet usage measurements recorded in November 2013 from Telecom Italia Call Data Records. This dataset serves as a gauge for the level of interaction between users and the mobile phone network. It includes fields such as SMS-in and out, Call-in and out, as well as Internet traffic activity. The SMS-in and SMS-out activities represent the quantity of received and sent SMS within a specified region and time period, and the same applies to Call activities. Meanwhile, Internet traffic activity denotes the volume of Call Detail Records (CDR) from phone subscribers globally. All these metrics serve as measures for network traffic. Therefore, we conduct the experiments using this dataset to validate our work, providing further substantiation for our exploration of the Metcalfe law family.

%We validated the aforementioned Metcalfe's Law and its variants using Milan dataset. It becomes evident that, with varying node quantities and diverse scenario selections, the traffic exhibits different functional relationships. We conducted random selections for different node quantities, considered their averages, and fitted corresponding functions. Remarkably, both Metcalfe's Law and its variants could be successfully fitted, as depicted in the Fig. \ref{pic-fit}. In the table below, we provide specific details regarding our data selection and parameter fitting for the functions. Combining our work with the findings \cite{zhang2023facebook,zhang2015tencent,briscoe2006metcalfe}, we demonstrate the rationality of these laws from an empirical validation perspective.
%
%From the conclusions drawn in Table \ref{tab-law-fit}, we can analyze distinct outcomes. Notably, when fitting a cubic function, the coefficient of the cubic term is significantly smaller than those of the quadratic and linear terms. However, when employing alternative functions for fitting, their performance does not match that of the cubic function. Hence, even though the coefficient of the cubic term is notably small, its impact on the function remains substantial. Consequently, when real-world scenarios exhibit changes in concavity, the cubic function demonstrates sufficient complexity to capture these variations effectively.

%We validated the aforementioned Metcalfe's Law and its variants using the Milan dataset. It becomes evident that, with varying node quantities and diverse scenario selections, the traffic exhibits different functional relationships. We conducted random selections for different node quantities, considered their averages, and fitted corresponding functions. Remarkably, both Metcalfe's Law and its variants could be successfully fitted, as depicted in Fig. \ref{pic-fit}. In Table \ref{tab-law-fit}, we provide specific details regarding our data selection and parameter fitting for the functions. Combining our work with the findings \cite{zhang2023facebook, zhang2015tencent, briscoe2006metcalfe}, we demonstrate the rationality of these laws from an empirical validation perspective.
%
%We selected several groups of experiment results with good fitting degrees for display. It can be observed that the Metcalfe family has been fitted well and exhibits good fits on average. In terms of data selection, to ensure statistical properties, we randomly selected data points for fixed days and a fixed number, performed statistics, and thus completed the data validation in this section.
%
%From the conclusions drawn in Table \ref{tab-law-fit}, we can analyze distinct outcomes. Notably, when fitting a cubic function, the coefficient of the cubic term is significantly smaller than those of the quadratic and linear terms. However, when employing alternative functions for fitting, their performance does not match that of the cubic function. Hence, even though the coefficient of the cubic term is notably small, its impact on the function remains substantial. Consequently, when real-world scenarios exhibit changes in concavity, the cubic function demonstrates sufficient complexity to capture these variations effectively.


We verify Metcalfe's Law and its variations using the Milan dataset, revealing distinct functional relationships in traffic under varying node quantities and diverse scenarios. Conducting random selections and averaging for different node quantities, we successfully fit Metcalfe's Law and its variants, as shown in Fig. \ref{pic-fit}. Detailed data selection and parameter fitting for the functions are provided in Table \ref{tab-law-fit}. By combining our results with previous findings \cite{zhang2023facebook, zhang2015tencent, briscoe2006metcalfe}, we assert the empirical validity of these laws.

We present the selected experiment results with favorable fitting degrees. It's evident that the Metcalfe's Law and its variants exhibit excellent fits on average. In terms of data selection, we ensure statistical robustness by randomly choosing data points for fixed days and a fixed number, performing rigorous statistical analyses for data validation.

%Analyzing the outcomes in Table \ref{tab-law-fit}, we note that, especially in cubic function fitting, the cubic term's coefficient is significantly smaller than those of the quadratic and linear terms. However, alternative functions do not match the performance of the cubic function. Despite the small coefficient of the cubic term, its impact on the function remains substantial. Thus, the cubic function, with its complexity, effectively captures variations when real-world scenarios present changes in concavity.

% Examining the results presented in Table \ref{tab-law-fit}, it is noteworthy, particularly in the fitting of cubic functions, that the coefficient of the cubic term is notably smaller than those of the quadratic and linear terms. However, alternative functions fail to achieve the same level of performance as the cubic function. Despite the seemingly small coefficient of the cubic term, its influence on the function remains significant. Consequently, the cubic function, with its inherent complexity, adeptly captures variations when real-world scenarios exhibit alterations in concavity.
From the conclusions drawn in Table \ref{tab-law-fit}, we can analyze distinct outcomes. Notably, when fitting a cubic function, the coefficient of the cubic term is significantly smaller than those of the quadratic and linear terms. However, when employing alternative functions for fitting, their performance does not match that of the cubic function. Hence, even though the coefficient of the cubic term is notably small, its impact on the function remains substantial. Consequently, when real-world scenarios exhibit changes in concavity, the cubic function demonstrates sufficient complexity to capture these variations effectively.


==> literature.tex <==
In this section, we provide a concise overview of our related works, which encompasses various laws related to Metcalfe's Law as well as their practical applications.

\subsection{Metcalfe's Law and Variants}
Wang et al. \cite{wang2023revisiting} revisited network value, providing detailed explanations of Sarnoff's Law, Metcalfe's Law, and Reed's Law. Next, we rake up and refine their overview.

Metcalfe's Law \cite{gilder1993metcalf} has become widely recognized as a concept synonymous with connectivity. According to this law, as the number of nodes in a network increases, the value of the network is proportional to the square of the number of nodes.
% Mathematically, Metcalfe's reasoning involves summing up all possible pairings between nodes, resulting in a network value of size $n$ expressed as $n(n-1)/2$, which can be simplified as being proportional to $n^2$.

%Reed's Law \cite{reed1999weapon} acknowledges the value of groups within a network rather than focusing solely on pairs. For instance, in a network consisting of four individuals, the value is not limited to pairings but also includes groups of three or even the entire group of four and more. By considering the possible combinations of groups of three and the complete group of four, the total number of subsets equals $2^n-n-1$. This approximation can be simplified as being proportional to $2^n$.
% 重写分组的概念
Reed's Law \cite{reed1999weapon} highlights the exponential increase in network value as the number of possible subgroups or communities formed within the network grows, i.e. $V\propto 2^n$. This concept underscores the significant impact of forming groups within a network, leading to exponential growth in network utility, collaboration, and information sharing. However, its application may vary depending on specific network contexts and the nature of interactions within subgroups. Overall, Reed's Law offers valuable insights into the exponential growth of network value through community formation.

Sarnoff's Law \cite{swann2002functional} examines the relationship between the aggregate value of television-mediated networks and the number of users. It reveals that the aggregate value of such networks is directly proportional to the number of nodes $n$, indicating that as the user count increases, the overall value of the network also increases linearly.

Odlyzko et al. \cite{briscoe2006metcalfe} raised the argument that Metcalfe's Law can often present overly optimistic estimations of network values. They propose that intuitively, the rate of network value growth should decrease as additional members join, aligning with the concept of \textit{diminishing returns} found in neoclassical economics. To capture this diminishing incremental value, they propose a model where the total value is calculated as $n\log n$, where future memberships contribute to a decreasing, yet still positive, growth in value.


\subsection{Applications on Metcalfe's Law}
% Metcalfe's Law has found numerous applications, serving as an explanatory model for the growth of various technologies, including phones, cell phones, faxes, web applications, and notably online social networks \cite{hendler2008metcalfe}. It has also been applied to digital blockchain networks to assess the value of digital currencies within those networks \cite{alabi2017digital}, as well as to analyze the price dynamics of Bitcoin \cite{peterson2018metcalfe,wheatley2019bitcoin}. The empirical evidence supporting Metcalfe's Law is substantial. Jun et al. \cite{jun2021how} conducted a study on duopoly competition among social network services (SNS), demonstrating that SNS adoption follows a polynomial function over time under both Metcalfe's Law and Reed's Law. They collected web traffic data from Facebook and Myspace for empirical analysis. In 2013, Robert Metcalfe \cite{metcalfe2013metcalfe}, the person after whom the law is named, utilized Facebook's historical data to demonstrate a good fit with Metcalfe's Law, with the network size defined as the number of monthly active users (MAUs) and network value defined as revenue. Zhang et al. \cite{zhang2015tencent} expanded Metcalfe's Law to analyze the data from Tencent, one of the largest social network companies in China, and found that Metcalfe's Law provided the best fit. However, in 2023, Zhang et al. \cite{zhang2023facebook} examined the latest data from Facebook and Tencent and discovered that a cube law ($V\propto n^3$) provided a better fit for the actual network values compared to Metcalfe's Law. While these studies offer empirical evidence supporting Metcalfe's Law, there remains a lack of comprehensive theoretical explanations.

% Metcalfe's Law has been widely applied as an explanatory model for the growth of various technologies, such as phones, faxes, web applications, and notably online social networks \cite{hendler2008metcalfe}. It has also found relevance in digital blockchain networks, assessing the value of digital currencies within those networks \cite{alabi2017digital}, and analyzing the price dynamics of Bitcoin \cite{peterson2018metcalfe,wheatley2019bitcoin}. Empirical evidence supporting Metcalfe's Law is substantial. Jun et al. \cite{jun2021how} studied duopoly competition among social network services (SNS) and demonstrated that SNS adoption follows a polynomial function, based on web traffic data from Facebook and Myspace. In 2013, Robert Metcalfe personally conducted a study \cite{metcalfe2013metcalfe} utilizing historical data from Facebook to demonstrate a strong correlation with Metcalfe's Law. In his research, he defined network size as the total count of monthly active users (MAUs), while network value was measured in terms of revenue. Zhang et al. \cite{zhang2015tencent} extended Metcalfe's Law to analyze data from Tencent and found that Metcalfe's Law provided the best fit. However, in 2023, Zhang et al. \cite{zhang2023facebook} examined the latest data from Facebook and Tencent, discovering that a cube law ($V\propto n^3$) better fitted the actual network values compared to Metcalfe's Law. While these studies offer empirical evidence supporting Metcalfe's Law, there remains a lack of comprehensive theoretical explanations.

Metcalfe's Law has been widely employed as an explanatory model for the growth of various technologies, spanning from traditional communication mediums like phones and faxes to modern web applications and, notably, online social networks \cite{hendler2008metcalfe}.  Its relevance extends to digital blockchain networks, where it evaluates the value of digital currencies within these decentralized systems \cite{alabi2017digital}.  Additionally, it has been instrumental in analyzing the price dynamics of cryptocurrencies like Bitcoin \cite{peterson2018metcalfe,wheatley2019bitcoin}.
The empirical validation supporting Metcalfe's Law is substantial and spans diverse domains.  For instance, Jun et al. \cite{jun2021how} conducted a study on duopoly competition among social network services (SNS), demonstrating that SNS adoption closely adheres to a polynomial function, leveraging web traffic data from platforms like Facebook and Myspace.
In 2013, Robert Metcalfe himself conducted a study \cite{metcalfe2013metcalfe} using historical data from Facebook, unveiling a robust correlation with Metcalfe's Law.  In this research, network size was quantified by the total count of monthly active users (MAUs), while network value was assessed in terms of revenue.  Further extending its applicability, Zhang et al. \cite{zhang2015tencent} applied Metcalfe's Law to analyze data from Tencent, and it emerged as the best-fitting model.
However, in 2023, Zhang et al. \cite{zhang2023facebook} reevaluated the most recent data from Facebook and Tencent, revealing that a cubic law ($V\propto n^3$) offered a more precise representation of actual network values compared to Metcalfe's Law.  Despite this empirical support, there is a notable gap in the availability of comprehensive theoretical explanations for these observed phenomena.

Moreover, there are numerous studies applying Metcalfe's Law in their respective domains. Starting from the Metcalfe's law family, Scala et al. \cite{scala2023explosive} investigated the governing patterns of network dynamics, analyzing their value dynamics from multiple perspectives, particularly emphasizing the explosive value of networks. Malik et al. \cite{milak2022years} suggested that the release of the Windows 95 operating system acted as a stimulant to Metcalfe's Law. The more people using Windows 95, the more valuable the network, establishing a positive cycle and laying the foundation for the symbiotic relationship between computing devices and networks. Ma et al. \cite{ma2023does} delved into the nonlinear relationship between Metcalfe's Law and the digitization of the green economy, affirming its relevance in the green transformation of Chinese cities. Addressing enterprise valuation challenges, DEVA method is proposed based on Metcalfe's Law to navigate the difficulties in recalculating costs \cite{tang5study}. Assif et al. \cite{assif2023fair} explored fairness in sharing total value among primary and secondary participants in crowdsourcing networks, incorporating empirical analysis. In the context of the digital transformation of Covid-19 healthcare, Roberto \cite{moro2023smart} considered network effects and applies Metcalfe's Law. Nowak et al. \cite{nowak2023social} integrated these laws into platform coordination for reshaping urban platforms. Ji et al. \cite{ji2023simple} introduced a Drop-type method based on them for low-quality image classification, adjusting neural network unit co-adaptation and predictive capabilities, effectively controlling neurons by randomizing parameter sharing ratios.

==> method.tex <==
% need modifications
\subsection{Value and Traffic Load for Network}
In a communication network, the sum of products of bits and the distances over which they are carried, i.e. the so-called \textit{traffic load}, is a valuable indicator of the network's transport capacity \cite{gupta2000capacity, jovicic2004upper}. In this paper, we mainly study the traffic load scaling of data dissemination in a type of generalized network.
\begin{defn}[Informal Definition of Network]\label{network}
	We consider the network composed of a random number of $N$ nodes distributed over a square region of a area $S:=n$,where $\mathbf{E}[N]=n$. To avoid border effects, we consider wraparound conditions at the network edges, i.e., the network area is assumed to be the surface of a Turos $\mathcal{O}$. To simplify the description, we assume that the number of nodes is exactly $n$, and denote the set of nodes by $\mathcal{V}=\{v_k\}_{k=1}^n$, without changing our results in order sense, \cite{15Franceschetti2007,peng2011heterogeneity,wang2012multicast}.
\end{defn}
 

In real life, social networks and the Internet of Things are two applications that are representative of the above definition. In social networks, users are treated as nodes. Each user can send data content, while other users can receive the desired data according to their interests. In the Internet of Things, objects are connected to each other via the Internet. Objects generate data through sensing devices, and other objects access this data on demand.

It seems that the values of networks are functions of traffic loads, i.e. $\mathbf{V}(n)=h(\mathbf{G}(N))$, where $\mathbf{V}(\cdot)$ denotes the value of networks, $\mathbf{G}(\cdot)$ denotes the traffic load of networks and $h(\cdot)$ is a non-decreasing function.  In Section \ref{Case}, we discuss the impact of the type of $h$ on the existing law as well as giving a realistic interpretation of the meaning.


 
 Considering a network, denoted by $\mathbb{N}$, consisting of $n$ users, denote the set of all users by $\mathcal{U}=\{u_i\}_{i=1}^n$; let a subset $\mathcal{S}=\{u_{\mathcal{S},k}\}_{k=1}^{n_s} \subseteq \mathcal{U}$ denote the set of all sources, where $|\mathcal{S}|=n_s$. 
 
Denote a Social-InterestCast session by an ordered pair $\mathbb{D}^{\mathrm{I}}_k=<v_{k}, \mathcal{I}_k>$, where $ v_{k} $ is the source and each element $ v_{k_{i}} $ in $\mathcal{I}_k=\{v_{k_i}\}_{i=1}^{d_k}$ is the nearest node to the corresponding $ p_{k_{i}} $ in $ \mathcal{A}^\mathrm{I}_k=\{p_{k_i}\}_{i=1}^{d_k} $, the random variable $d_{k}$ denotes the number of potential destinations for session $\mathbb{D}^{\mathrm{I}}_k$, i.e., the neighbor of $v_{k}$ who are interested in the message from $v_{k}$ in this session.

We introduce two key conceptions: \textit{data arrival process for users and transport distance of messages}.
\subsubsection{Data Arrival Process for Users}
\textbf{Individual Data Arrival Process.} The temporal behavior of messages arriving at a user in an OSNs has been addressed by analyzing some real-life OSNs. For example, Perera et al. \cite{perera2010twitter} developed a software architecture that uses a Twitter application program interface (API) to collect the tweets sent to specific users. They indicated that the arrival process of new tweets to a user can be modeled as Poisson Process. In this work, we just make it as an empirical argument for assuming the data arrival for a user as a data source to follow a Poisson Process. We define a rate vector
\begin{equation}
	\label{poisson rate}
	\Lambda_{\mathcal{S}}=(\lambda_{\mathcal{S},1}, \lambda_{\mathcal{S},2}, \cdots, \lambda_{\mathcal{S},n_s})
\end{equation}
where $\lambda_{\mathcal{S},k}$ is the rate of the Poisson Process ar user $u_{\mathcal{S},k}$ (for $k=1, 2, \cdots, n_s$), and is called \textit{data arrival/generating rate}. 
% Here, we make a reasonable and practical assumption that $\lambda_{\mathcal{S},k}=\Theta(1)$ for $k=1, 2, \cdots, n_s$.

% \textbf{Data Arrival Rate Distribution.} The results of interest in this paper fall within the scope of scaling laws issue. Therefore, although in practice, the individual data arrival/generating process may depend on many factors such as the user's location, it is appropriate  to note at this point that the specific distribution of data arrival rate has no impact on the results (in order sense) as long as it holds that $\lambda_{\mathcal{S},k}=\Theta(1)$ for $k=1,2,\cdots,n_{\mathcal{S}}$. This is the reason why we do not make an intensive study of the specific distribution of data arrival rates.

\subsubsection{Transport Distance of Messages}

\textbf{Transport Distance of Messages:}
For a given transmission scheme in a given  OSN $\mathbb{N}$, say $\mathbf{S}_\mathbb{N}$, define a vector
\[\mathbf{D}_{\mathcal{S}}(\mathbf{S}_\mathbb{N})=\left(d_{\mathcal{S},1}(\mathbf{S}_\mathbb{N}), d_{\mathcal{S},2}(\mathbf{S}_\mathbb{N}), \cdots, d_{\mathcal{S},n_s}(\mathbf{S}_\mathbb{N}) \right),\]
where
$d_{\mathcal{S}, k}(\mathbf{S}_\mathbb{N})$ represents the \emph{transport distance} over which the message for session $\mathbb{D}_{\mathcal{S}, k}$ is successfully transported from the source $u_{\mathcal{S}, k}$ to all destinations.
Clearly, the transport distance depends on the specific architectures of carrier communication networks and transmission strategies.





%\subsubsection{Transport Load for OSNs}\label{subsec-transportload}


\textbf{Transport Load and Transport Complexity:}
In the OSN $\mathbb{N}$, given a specific carrier communication network, define the transport load for a dissemination session, say $\mathbb{D}_{\mathcal{S}, k}$, as
\[
\widetilde{\mathbf{L}}_{\mathbb{N},\mathcal{S}}(\mathbb{D}_{\mathcal{S}, k})=\lambda_{\mathcal{S},k} \cdot d_{\mathcal{S},k}(\mathbf{S}_\mathbb{N}).\] Furthermore, the aggregated transport load for dissemination sessions from all sources in  $\mathcal{S}$ can be  defined as
\begin{equation}\label{equ-transport-load}
	\mathbf{L}_{\mathbb{N},\mathcal{S}}= \min\nolimits_{\mathbf{S}_\mathbb{N}\in \mathbb{S}} \mathbf{\Lambda}_{\mathcal{S}}  \ast \mathbf{D}_{\mathcal{S}}(\mathbf{S}_\mathbb{N}),
\end{equation}
where $\mathbb{S}$ is the set of all feasible transmission schemes, and $\ast$ is an inner product.


Based on the definition of transport load, we further introduce the \emph{feasible transport load}.

\begin{defn}[Feasible Transport Load]\label{feasible-traffic-load}
	For a social data dissemination with a set of social sessions $\mathbb{D}_{\mathcal{S}}=\{\mathbb{D}_{\mathcal{S}, k}\}_{k=1}^{n}$, we say that the network transport load
	$\mathbf{L}_{\mathbb{N},\mathcal{S}}$
	is \emph{feasible} if and only if
	there exists an appropriate transmission scheme with a communication deployment, denoted  by $\mathbf{S}_\mathbb{N}$,
	such that
	it holds that $\mathbf{D}_{\mathcal{S}}(\mathbf{S}_\mathbb{N}) * \mathbf{\Lambda}_{\mathcal{S}}  \leq \mathbf{L}_{\mathbb{N},\mathcal{S}}$ ensuring that the network throughput of $\mathbf{\Lambda}_{\mathcal{S}} $ is achievable.
\end{defn}

Based on the definition of feasible transport load, we finally define the \emph{transport complexity}.
\begin{defn}[Transport Complexity]\label{tansmission-complexity}
	We say that the \emph{transport complexity} of the class of random social data dissemination $\mathbb{D}_{\mathcal{S}}$ is
	of order $ \Theta(f(n)) $ bit-meters per second
	if there are deterministic constants $ c_1 > 0 $ and $ c_2 < \infty $ such that:
	There exists a communication architecture $\mathbb{N}$ and corresponding transport schemes such that
	\begin{equation*}
		\lim_{n\longrightarrow\infty} \Pr (\mathbf{L}_{\mathbb{N},\mathcal{S}} = c_1 \cdot f(n) \mbox{ is feasible}) = 1,
	\end{equation*}
	and  for any possible communication architectures and transport schemes, it holds that:
	\begin{equation*}
		\liminf_{n\longrightarrow\infty} \Pr(\mathbf{L}_{\mathbb{N},\mathcal{S}} = c_2  \cdot f(n) \mbox{ is feasible}) <1.
	\end{equation*}
\end{defn}

\section{Model of Social-InterestCast}\label{section-Network Model}





For each session, the geographical distribution of the source and destination(s) plays a key role in generating the transport load.
So it is critical to analyze  the correlation between the spatial distribution of sessions and geographical distribution of users in the networks.

To address this issue, we propose a four-layered model,  consisting of
the  physical layer,  interaction layer, content layer, and  session layer, as illustrated in Figure \ref{fig-4-layer-archi}.

\subsection{Four-Layered System Model}




\subsubsection{Physical Layer- Physical Network Deployment}
The deployment of so-called physical network can be divided into two parts. The first is the geographical distribution of the nodes. The second is the communication architecture of  the carrier network.


\textbf{Geographical Distribution of Social Users:} 
We make a compromise in the generality and practicality of the geographical distribution of nodes in networks,
in order to concentrate on clarifying the impacts of content on the session formation.
Specifically, we follow the setting where all nodes are distributed according to a homogeneous Poisson point process, taking no account of the inhomogeneous property of the uneven population distribution in real-life networks.
The derived results are expected to serve as the basis for investigating more realistic scenarios under
the more practical but complex deployment models, such as the Clustering Random Model (CRM) according to the shotnoise Cox process \cite{alfano2009capacity,1wanglaoshisocial} and Multi-center Gaussian Model
(MGM) in \cite{mgm2012}.


\textbf{Communication Architecture of  Carrier Network:}
For online social networking services, we state that the carrier network is indeed the mobile Internet.
This means that there is hardly a uniform communication architecture, e.g., centralized or distributed network architecture, practically characterizing the architecture of a real-world carrier network for our networks.
This is also the reason why we only provide the lower bound on transport complexity for the optimal communication architecture of carrier network.

\subsubsection{Social Layer- Social Relationship}
Based on \cite{mobihoc2014}, we improve the density-aware relationship formation model in our work, defined as \emph{population-distance-based model}.  %(P-SF Model)
%Due to limited space, we cannot include the detailed description of this model. For the readability,we introduce the model by replacing with some notions in Appendix A of our technical report \cite{dropboxmobihoc2016}.
In \cite{mobihoc2014}, Wang et al. provided a numerical evaluation for this social model based on a Brightkite users' dataset \cite{gowalla2007}.
Before deciding to follow this social model, we complement an evaluation based on another dataset from \cite{gowalla2007},
i.e.,  a Gowalla users' dataset.
For the completeness, we include the evaluations based on these two datasets in Appendix \ref{appendix-sec-evaluation}.

%
%\section{Population-Distance-Based Social Formation Model}\label{appendix-relevant-results}
Let $\mathcal{D}(u, r)$ denote the disk centered at a node $u$ with radius $r$ in the deployment region $\mathcal{O}$, and let
$N(u, r)$ denote the number of nodes contained in  $\mathcal{D}(u, r)$.
Then, for any two nodes, say $u$ and $v$, we can define the \emph{population-distance} from $u$ to $v$ as $N(u, |u-v|)$,
where $|u-v|$ denotes the Euclidean distance between node $u$ and node $v$.


Now, the improved population-distance-based model is showed as follows:
For a node $v_k\in \mathcal{V}$,
construct its neighboring set $\mathcal{F}_k$ of $q_k$ ($q_k\geq 1$) nodes/friends by the following three procedures.

$\rhd$ \textbf{Zipf's Degree Distribution of Social Relationships:}
%\subsection{Zipf's Degree Distribution of Social Relationships}
Assume that the number
of neighbors (or followers) of a particular node $v_k\in \mathcal{V}$, denoted by  $q_k$, follows a  Zipf's
distribution \cite{manning1999foundations}, i.e.,
\begin{equation}\label{equ-zip-destinations}
	\Pr(q_k=l)={\left(\sum\nolimits_{j=1}^{n-1}j^{-\gamma}\right)^{-1}} \cdot {l^{-\gamma}}.
\end{equation}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
From Eq.(\ref{equ-zip-destinations}), we can observe that the degree distribution above depends on the specific network size (the number of nodes $n$).
Then, we give a numerical evaluation based on Gowalla dataset \cite{gowalla2007} for the Zipf's degree distribution in Appendix \ref{appendix-ddobu234324}.





We notice that the correlation between the nodes' degree distribution and graphical distribution should not be neglected, although we simplify it in this work.


$\rhd$ \textbf{Population-Distance-Based Formation of Social Relationships:}
%\subsection{Population-Distance-Based Formation of Social Relationships} We make the position of node $v_k$ as the \emph{reference point} and choose  $q_k$ \emph{points} independently on the torus region $\mathcal{O}$ according to a  probability distribution with
density function:
\begin{equation}\label{equ-social-distribution}
	f_{v_k}(X) = \Phi_k(S, \beta) \cdot \left ( \mathbf{E}[N(v_k, |X-v_k|)] +1 \right )^{-\beta} ,
\end{equation}
where the random variable $X:=(x,y)$ denotes the position of a selected point in the deployment region,
%$|X-v_k|$ denotes the Euclidean distance  between point $X$ and node $v_k$,
and $\beta\in [0, \infty)$ represents the clustering exponent of closure degree; the coefficient $\Phi_k(S, \beta)>0$  depends on $\beta$ and $S$ (the area of deployment region) and it satisfies:
\begin{equation}\label{equ-formation-completeness-condition}
	\Phi_k(S, \beta) \cdot \int_{\mathcal{O}} \left ( \mathbf{E}[N(v_k, |X-v_k|)] +1 \right )^{-\beta} d X =1.
\end{equation}

$\rhd$ \textbf{Nearest-Principle Position of  Followers:}
%\subsection{Nearest-Principle Position of Friends/ \\Followers:}
Let $\mathcal{A}_k=\{p_{k_i}\}_{i=1}^{q_k}$ denote the set of these $q_k$ points.
Let $v_{k_i}$ be
the nearest node to  $p_{k_i}$, for $1 \leq i \leq q_k$ (ties are broken randomly). Denote the set of these $q_k$ nodes by
$\mathcal{F}_k=\{v_{k_i}\}_{i=1}^{q_k}$.
%Please see the illustration in Fig.\ref{fig-social-formation}.
We call point $p_{k_i}$ the \emph{anchor point} of $v_{k_i}$, and define a set
$\mathcal{P}_k:= \{v_k\} \cup \mathcal{A}_k.$









Throughout this paper, we use $\mathbb{P}(\gamma, \beta)$ to denote the population-distance-based model. Here, $\gamma$ and
$\beta$ denote the clustering exponents of centrality degree and closure degree \cite{1wanglaoshisocial}, respectively.
For their detailed meanings, please refer to Eq.(\ref{equ-zip-destinations}) and Eq.(\ref{equ-social-distribution}), respectively.



\subsubsection{Content Layer- User-Content Interest Mapping}
In this work, we focus on the case where a node only read/watch the messages within his/her requirements.
Then, modeling the mapping between nodes and content is the first critical step for the final generation of traffic sessions.
The basic idea for this issue is to build the attractiveness links from users to messages according to the similarity
of nodes' requirements to the semantics of messages.
Here, we dig the node's requirements by abstracting the topics of all its posted messages.




\subsubsection{Session Layer- Data Traffic Session}\label{subsec-social-session-layer}
When observing nodes' behaviour in networks, there exists a significant feature of traffic session, i.e.,
the nodes' intrinsic selectivity and active choice are often indispensable for forming the sessions.
For all the common traffic patterns in networks, we focus on a typical data dissemination, called SocialCast, which can be divided into two successive phases: \emph{Passive Phase} and \emph{Active Phase}.
In the passive phase, a source node holding a message sends self-appointedly the digest of this message to all his followers. The followers passively receive this digest.
This process just acts like a broadcast in all the followers of this source node.
We call this process \emph{Social-BroadCast} by following an existing conception.
In the active phase, according to the requirements, a node will autonomously determine whether to receive the complete message based on the digest of a message from which its follows.
We define such an selectivity-driven dissemination process \emph{Social-SelectivityCast}.
The Social-SelectivityCast is defined by taking into account specific user interests and their effects on session generation.
Since the Social-BroadCast session pattern had been investigated in \cite{mobihoc2014}, then our focus in this work is Social-SelectivityCast.






\subsection{Social-SelectivityCast}\label{social_selectivitycastmodel}
In real-life OSNs, we find that there exists naturally a common phenomenon: When a user broadcasts messages to others, the number of potential destinations is depending on underlying relationships among users (both the source and destinations). For a delivered message, to explore the characteristics of source user and final destinations, we begin with studying relationships between users and messages. Then, we find that if a user broadcasts a message characterized by several words (an abstract) in his Facebook, only the users whose interests are consistent with the topic of the message can be the final destinations. We say that this behavior occurs due to an underlying \emph{user-message mapping} between user set and message set. For such type of  session and combining the networks we set in definition \ref{network}, we call it \emph{Social-SelectivityCast}, which is different than Unicast in \cite{02Gupta2000} and Social-BroadCast in \cite{mobihoc2014}. 


\subsubsection{Modeling Social-SelectivityCast}\label{model-for-interestcast}
The observations above turn out that the distribution of session destinations for Social-SelectivityCast follows approximately a Zipf's distribution. To be specific, for a source node $v_{k}$, based on the dependency among neighbors' decisions and the attractivity difference of message content, we make a reasonable assumption that the number of destinations follows a Zipf's distribution whose parameters depend on the friendship degree of $v_{k}$, i.e,
\[\mathrm{Pr}(d_{k}=d|q_{k}=l)={\left(\sum\nolimits_{m=1}^{l}m^{-\varphi_{k}}\right)^{-1}} \cdot  d^{-\varphi_{k}}, \]
where $ d_{k} $ is the number of session destinations of a session initiated by $v_{k}$ and $ \varphi_k\in[0,\infty) $ is the exponent of data dissemination. Here, for problem simplification, we first study the particular case where all $\varphi_{k}$ are assumed to be an identical value $ \varphi $.

%For Social-InterestCast, it is a more common session pattern when comprehensively considering the user behaviour in real-world OSNs and the interest-driven characteristic of OSNs.

In the following section, we mainly study this data dissemination and give the corresponding results for transport complexity.


\begin{table}[t] \renewcommand{\arraystretch}{1.6}
	\caption{Notations for Exponents}
	\label{tab-exponent-notation} \centering
	
	\scalebox{1.0}{    \begin{tabular}{l|p{6.5cm}}
			\hline Notation & Definition
			\\
			\hline \hline
			%$\mu_{\mathrm{s}} \in [0,1] $         &  scaling exponent of deployment region
			%\\
			%\hline
			%$\mu_{\mathrm{c}} \in [0,1] $ &   density exponent of centers
			%\\
			%\hline
			$\alpha \in [0,\infty)$  & clustering exponent of node distribution
			\\
			\hline
			
			$\beta \in [0, \infty)$          & clustering exponent of closure degree
			\\
			\hline
			
			$\gamma \in [0,\infty)$  & clustering exponent of centrality degree
			\\
			\hline
			
			$\varphi \in [0, \infty)$  & exponent of data dissemination
			\\
			\hline
		\end{tabular}
	}
\end{table}



\section{Bound on Transport Complexity for Social-InterestCast}\label{section-social-dissemination-systeme-setting}\
% The Social-InterestCast is the focus of this work for the fact that the transport load for Social-BroadCast had been investigated in \cite{mobihoc2014}. In this section, we derive the lower bound on transport complexity for Social-InterestCast.




\subsection{Social-InterestCast Sessions}\label{interestcast-session}

We call point $p_{k_{i}}$ the \emph{anchor point} of $v_{k_{i}}$, and define a set $\mathcal{P}^\mathrm{I}_{k} := \{v_{k}\} \cup \mathcal{A}^\mathrm{I}_k$. Then, we can get the following lemma.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{lem}\label{lem-EMST-B-D} For a Social-InterestCast session $\mathbb{D}^{\mathrm{I}}_k$, when $ d_{k}=\omega(1) $, with probability $1$, it holds that
	\begin{equation*}
		|\EMST(\mathcal{A}^\mathrm{I}_k)|=\Theta(L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)),
	\end{equation*}
	and then
	\begin{equation*}
		|\EMST(\mathcal{P}^\mathrm{I}_{k})|=\Omega(L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)),
	\end{equation*}
	where $\EMST(\cdot)$ denotes the Euclidean minimum spanning tree over a set,
	\begin{equation}\label{eq-L-P-beta-9765}
		L^\mathrm{I}_{\mathcal{P}}(\beta, d_k) = \left\{
		\begin{array}{ll}
			\Theta\left( \sqrt{d_k} \right)  , &  \beta>2;  \\
			\Theta\left(\sqrt{d_k} \cdot \log n  \right), &  \beta=2;  \\
			\Theta\left(\sqrt{d_k} \cdot n^{1-\frac{\beta}{2}} \right)  , & 1< \beta < 2;  \\
			\Theta\left(\sqrt{d_k} \cdot \sqrt{\frac{n}{\log n}} \right) , &  \beta=1;  \\
			\Theta\left(\sqrt{d_k} \cdot \sqrt{n} \right)  , &  0\leq\beta <1.
		\end{array}
		\right.
	\end{equation}
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\end{lem}
\begin{proof}
	With probability $1$, it holds that
	\begin{center}
		$|\EMST(\mathcal{A}^\mathrm{I}_k)|=\Theta(L^\mathrm{I}_{\mathcal{P}}(\beta, d_k))$ for $d_k=\omega(1)$,
	\end{center}
	where $L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)$ is defined in Eq.(\ref{eq-L-P-beta-9765}). Combining with the fact that \[|\EMST(\mathcal{P}^\mathrm{I}_{k})|\geq |\EMST(\mathcal{A}^\mathrm{I}_k)|,\] then, we get that
	\begin{equation*}
		|\EMST(\mathcal{P}^\mathrm{I}_{k})|=\Omega(L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)).
	\end{equation*}
	Then, our focus turns to the derivation of $ L^\mathrm{I}_{\mathcal{P}}(\beta, d_k) $. Based on the value of $ \beta $, we have:
	
	
	
	
	(1) When $ 0 \leq\beta <1 $,
	\begin{equation*}
		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)} dX =  \Theta\left(n^{\frac{\beta-1}{2}} \cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right)
	\end{equation*}
	$~~~~~~~~~~~~~~~~~~~~~~~= \Theta\left(n^{\frac{\beta-1}{2}} \cdot n^{1-\frac{\beta}{2}}\right) = \Theta\left(\sqrt{n}\right) $.
	
	
	(2) When $ \beta=1 $,
	\begin{equation*}
		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left(\frac{1}{\sqrt{\log n}}\cdot \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{1}{2}}}\right)
	\end{equation*}
	$~~~~~~~~~~~~~~~~~~~~~~~= \Theta\left(\frac{1}{\sqrt{\log n}} \cdot \sqrt{n}\right) = \Theta\left(\sqrt{\frac{n}{\log n}}\right) $.
	
	(3) When $ \beta>1 $,
	\begin{equation*}
		\int_{\mathcal{O}}\sqrt{f_{X_0}(X)}dX = \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right).
	\end{equation*}
	
	Especially,
	
	when $ 1<\beta<2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right) = \Theta\left(n^{1-\frac{\beta}{2}}\right) $;
	
	when $ \beta=2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)}\right) $=$ \Theta\left(\log n\right) $;
	
	when $ \beta>2 $, $ \Theta\left( \int_{\mathcal{O}}\frac{dX}{\left(|X-X_{0}|^{2}+1\right)^{\frac{\beta}{2}}}\right) $=$ \Theta\left(1\right) $.
	
	Combining with all cases above, we complete the proof.
\end{proof}



\subsection{Main Results on Transport Complexity}\label{Z-D-result-interestcast}
The following Theorem \ref{Z-D-thm-transport-load-on-sessions} demonstrates a lower bound on transport complexity for OSN $\mathbb{N}$ as follows.
\begin{thm}\label{Z-D-thm-transport-load-on-sessions}
	Let $\mathrm{L}_{\mathbb{N}}^{\mathrm{I}}$ denote the transport complexity for all data dissemination sessions in OSN $\mathbb{N}$.
	For the Social-InterestCast with the Zipf's distribution, it holds that
	\begin{equation*}
		\mathrm{L}_{\mathbb{N}}^{\mathrm{I}}=\Omega\left(G\left(\beta, \gamma, \varphi\right)\right),
	\end{equation*}
	where the value of $ G\left(\beta, \gamma, \varphi\right) $, presented in Table \ref{G-tab-total} in Appendix \ref{lower-bound-G},
	% of our technical report \cite{dropboxmobihoc2016},
	depends on  the clustering exponents of friendship degree $\gamma$, friendship formation $\beta$ and dissemination pattern $ \varphi $.
\end{thm}





\subsubsection{Proof of Theorem \ref{Z-D-thm-transport-load-on-sessions}}\label{proof-Z-D-transmission-complexity}
The bound on the transport complexity depends on the lower bounds on $ \sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}^\mathrm{I}_k)| $, which we compute in the following lemma.
\begin{lem}\label{lem-delta-0-all-est} For all Social-InterestCast sessions $ \{\mathbb{D}^{\mathrm{I}}_k\}_{k=1}^{n} $ with the Zipf's distribution, with high probability, the lower bounds on $ \sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}^\mathrm{I}_k)| $ are presented in Table \ref{tab-lower-bound-EMST} in Appendix \ref{lower-bound-E}.
	% of our technical report \cite{dropboxmobihoc2016}.
	
\end{lem}
\begin{proof}
	Denote the number of users with $ l $ destinations as $ T_{l} $, to simplify the proof, we let
	\begin{equation*}
		T_{l}  =  n\cdot\mathrm{Pr}(q_{k}=l)  = n\cdot{\left(\sum\nolimits_{j=1}^{n-1}j^{-\gamma}\right)^{-1}} \cdot (l)^{-\gamma}.
	\end{equation*}
	According to laws of larger numbers (LLN), it has no impact on the analysis process of issue in order sense.
	For all sessions $\{\mathbb{D}^{\mathrm{I}}_k\}_{k=1}^{n}$, we define two sets:
	\begin{equation*}
		\mathcal{K}^{1}:=\{k|q_{k}=\Theta(1)\}, \mathcal{K}^{\infty}:=\{k|q_{k}=\omega(1)\}.
	\end{equation*}
	Then, it follows that
	\begin{equation}\label{Transport-sum}
		\sum\nolimits_{k=1}^{n}|\EMST(\mathcal{P}^\mathrm{I}_k)|  = \widehat{{\Sigma}}^{1} + \widehat{{\Sigma}}^{\infty},
	\end{equation}
	where
	\begin{equation*}
		\widehat{{\Sigma}}^{1} = \sum_{k\in\mathcal{K}^{1}}|\EMST(\mathcal{P}^\mathrm{I}_k)|,
		\widehat{{\Sigma}}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}}|\EMST(\mathcal{P}^\mathrm{I}_k)|.
	\end{equation*}
	We first address the part of $\widehat{{\Sigma}}^{1}$. Since for $q_{k}=\Theta(1)$, it holds that
	\[ |\EMST(\mathcal{P}^\mathrm{I}_k)|=\Theta(|X-v_{k}|). \]
	Then we have
	$ \widehat{{\Sigma}}^{1}=\sum\nolimits_{k\in\mathcal{K}^{1}}|X-v_{k}|. $
	For $ k\in\mathcal{K}^{1} $, we define a sequence of random variables
	$ \phi^{1}_{k}:=|X-v_{k}|/\sqrt{n} $,
	which have finite meaning as follows:
	$ E[\phi^{1}_{k}] = E[|X-v_{k}|]/\sqrt{n},$
	where $E[|X-v_{k}|]$ is given in Lemma 5 of \cite{mobihoc2014}.
	Then, according to Lemma \ref{lem-growthsteel}, with probability $1$, it holds that
	\[ \widehat{{\Sigma}}^{1}=\Theta \left(\sqrt{n}\cdot\sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k}\right),\]
	and
	\begin{equation*}
		\sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k} / |\mathcal{K}^{1}|=\Theta(E\left[|X-v_{k}|/\sqrt{n}\right]),
	\end{equation*}
	where $ |\mathcal{K}^{1}| $ denotes the cardinality of set $ \mathcal{K}^{1} $.
	Therefore,
	\[ \sum\nolimits_{k\in\mathcal{K}^{1}}\phi^{1}_{k} = \Theta\left(|\mathcal{K}^{1}|\cdot E\left[|X-v_{k}|/\sqrt{n}\right]\right).\]
	Then, by Lemma \ref{lem-Kolmogorov-slln}, with probability $1$, it holds that
	\begin{equation}\label{Transport-for-k-1}
		\widehat{{\Sigma}}^{1}=\Theta\left(|\mathcal{K}^{1}| \cdot E[|X-v_{k}|] \right).
	\end{equation}
	Next, we consider $ \widehat{{\Sigma}}^{\infty} $. By introducing anchor points, all random variables $ |\EMST(\mathcal{P}^\mathrm{I}_k)| $ with $k \in \mathcal{K}^{\infty}$ are independent. For users with friends number in $ \mathcal{K}^{\infty} $, we define two sets:
	\begin{equation*}
		\mathcal{K}^{\infty}_{1} = \{k|d_{k} = \Theta\left(1\right)\}, \mathcal{K}^{\infty}_{\infty} = \{d_{k} = \omega\left(1\right)\}.
	\end{equation*}
	Then, it follows that
	\begin{equation}\label{Transport-for-k-wuqiong}
		\widehat{{\Sigma}}^{\infty} =  \widehat{{\Sigma}}_{1}^{\infty} + \widehat{{\Sigma}}_{\infty}^{\infty},
	\end{equation}
	where
	\begin{equation*}
		\widehat{{\Sigma}}_{1}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}_{1}}|\EMST \left(\mathcal{P}^\mathrm{I}_k\right)|,
		\widehat{{\Sigma}}_{\infty}^{\infty} = \sum_{k\in\mathcal{K}^{\infty}_{\infty}}| \EMST \left(\mathcal{P}^\mathrm{I}_k\right)|.
	\end{equation*}
	We first consider the $ \mathcal{K}^{\infty}_{1} $. For $ d_{k} = \Theta\left(1\right) $, the order of $ \widehat{{\Sigma}}_{1}^{\infty} $ is lower than that of $ \widehat{{\Sigma}}^{1} $. For the final summation, the specific value of $ \widehat{{\Sigma}}_{1}^{\infty} $ is relatively infinitesimal.
	
	Next, we consider $ \mathcal{K}^{\infty}_{\infty} $.
	According to Lemma \ref{lem-EMST-B-D}, with probability $1$, it holds that
	\begin{equation*}
		|\mathrm{EMST\left(\mathcal{P}^\mathrm{I}_k\right)}| = \Omega\left(L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)\right),
	\end{equation*}
	where $L^\mathrm{I}_{\mathcal{P}}(\beta, d_k)$ is defined in Eq.(\ref{eq-L-P-beta-9765}). And using LLN, with probability $1$, it follows that
	\begin{equation}\label{Transport-for-d-wuqiong}
		\widehat{{\Sigma}}_{\infty}^{\infty} \geq \sum\nolimits_{l=2}^{n-1} \sum\nolimits_{d=1}^{l} T_{l} \cdot \mathrm{Pr}(d_{k}=d|q_{k}=l) \cdot L^\mathrm{I}_{\mathcal{P}}\left(\beta,d\right).
	\end{equation}
	Combining with Eq.(\ref{Transport-sum}), Eq.(\ref{Transport-for-k-1}), Eq.(\ref{Transport-for-k-wuqiong}) and Eq.(\ref{Transport-for-d-wuqiong}), we complete the proof of Lemma \ref{lem-delta-0-all-est}.
\end{proof}


Next, we begin to prove Theorem \ref{Z-D-thm-transport-load-on-sessions}. Since
\begin{equation*}
	\sum_{k=1}^{n} d_{k} = \Theta\left(\sum_{l=1}^{n-1} \sum_{d=1}^{l} T_{l} \cdot \mathrm{Pr}(d_{k}=d|q_{k}=l) \cdot d \right),
\end{equation*}
we derive that $ \sum\nolimits_{k=1}^{n} d_{k} = W\left(\gamma, \varphi\right),$ where $ W\left(\gamma, \varphi\right) $  is described in  Table \ref{tab-W-gamma-varphi}.
\begin{table}[t]
	\renewcommand{\arraystretch}{1.2}
	\centering
	\caption{The Number of All Destinations, $W\left(\gamma, \varphi\right)$}
	\label{tab-W-gamma-varphi}
	\scalebox{0.85}
	{
		%\begin{tiny}
		\renewcommand\arraystretch{1.2}
		\begin{tabular}{|p{2cm} ||p{5.9cm}|}
			\hline
			$\varphi$ & $ W\left(\gamma, \varphi\right) $\\
			\hline
			\hline
			$\varphi>2$ &
			$ \Theta(n) $  , $ \gamma\geq0.$ \\
			\hline
			$\varphi=2$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \gamma >1; \\
				\Theta(n \cdot \log n) , &  \gamma=1;  \\
				\Theta(n \cdot \log n)  , &  0\leq\gamma<1.
			\end{array}
			\right. $ \\
			\hline
			$1<\varphi<2$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n) , &  \gamma>3-\varphi;  \\
				\Theta(n \cdot \log n) , &  \gamma=3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi})  , &  1<\gamma<3-\varphi; \\
				\Theta(n^{3-\varphi} / \log n) , &  \gamma=1; \\
				\Theta(n^{3-\varphi})  , &  0\leq\gamma<1.
			\end{array}
			\right. $ \\
			\hline
			$\varphi=1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \gamma\geq2;\\
				\Theta(n^{3-\gamma}/ \log n) , &  1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , &  \gamma=1;  \\
				\Theta(n^{2}/ \log n)  , &  0\leq\gamma<1.
			\end{array}
			\right. $ \\
			\hline
			$0\leq\varphi<1$ &
			$\left\{
			\begin{array}{ll}
				\Theta(n)  , &  \gamma>2; \\
				\Theta(n \cdot \log n)  , &  \gamma=2; \\
				\Theta(n^{3-\gamma})  , &  1<\gamma<2; \\
				\Theta(n^{2}/\log n) , &  \gamma=1;  \\
				\Theta(n^{2})  , &  0\leq\gamma<1.
			\end{array}
			\right. $ \\
			\hline
		\end{tabular}
		%\end{tiny}
	}
\end{table}
Additionally, for all $ v_{k} \in \mathcal{V}$ that launch sessions,
\begin{equation*}
	E[| v_{k_{i}} - p_{k_{i}} |] = \Theta\left( \int_{0}^{\sqrt{n}} x \cdot e^{-\pi \cdot x^{2}}dx \right).
\end{equation*}
That is, \[ E[| v_{k_{i}} - p_{k_{i}} |] = \Theta \left(1\right). \]
Therefore, according to Lemma \ref{lem-Kolmogorov-slln}, with probability $1$, it follows that
%it holds that
%\[\frac{\sum_{i=1}^{d_{k}} |v_{k_{i}}-p_{k_{i}}|}{d_{k}}=\Theta(1),\]
% i.e.,
% $ \sum_{i=1}^{d_{k}} |v_{k_{i}}-p_{k_{i}}| = \Theta(d_{k}) $.
%   Then
\begin{equation}\label{Length-Anchor-Friends}
	\sum\nolimits_{k=1}^{n} \sum\nolimits_{i=1}^{d_{k}} |v_{k_{i}}-p_{k_{i}}| = \Theta \left(\sum\nolimits_{k=1}^{n} d_{k}\right) = \Theta\left(W\left(\gamma, \varphi\right)\right).
\end{equation}
Combining with Lemma \ref{lem-delta-0-all-est}, for all Social-InterestCast sessions $\mathbb{D}^{\mathrm{I}}_k$, $ k = 1, 2, ..., n $, with high probability, it holds that
\[ \sum\nolimits_{k=1}^n| \mathrm{EMST}(\mathbb{D}^{\mathrm{I}}_k) | = \Omega \left(G\left(\beta, \gamma, \varphi\right)\right) ,
\]
where $G\left(\beta, \gamma, \varphi\right)$ is provided in Table \ref{G-tab-total} in Appendix \ref{lower-bound-G}.
% of our technical report \cite{dropboxmobihoc2016}.
Then, we complete the proof of Theorem \ref{Z-D-thm-transport-load-on-sessions}.



%\subsubsection{Intuitive Results -Special Cases of Our Results}\label{special-case-results}
\subsubsection{How to Understand Our Results}\label{special-case-results}
For space limit, we contain the complete results in Appendix \ref{our-reslts}, i.e., Table \ref{G-tab-total} and Table \ref{tab-lower-bound-EMST}.
Our results in Table \ref{G-tab-total} is depended on three parameters, i.e., $\gamma$, $\beta$, and $\varphi$. The final results is in the range $\left[\Theta(n), \Theta(n^{2})\right]$, when $\gamma$, $\beta$, and $\varphi$ have different values, respectively.

For Table \ref{tab-lower-bound-EMST} and Table \ref{G-tab-total}, they are too complex to provide a clear insight on the results.
To facilitate the understanding of our results, we choose a part of results and make them visualized. Figure \ref{fig-result-gamma3/2} illustrates the results under $1<\beta<2$ and $1<\varphi<\frac{3}{2}$:

\subsubsection{Explanation of Results}\label{Z-D-subsub-explaination-social-dissemination-results}
We mainly discuss the impacts of the clustering exponent of dissemination pattern $\varphi$ on the transport complexity with Social-InterestCast in this subsection. Our result demonstrates that the lower bound on transport complexity for Social-InterestCast is in the range $\left[\Theta(n), \Theta(n^2)\right]$ with the clustering exponents of friendship degree $\gamma$, friendship formation $\beta$, and dissemination patter $\varphi$.
An intuitive explanation is as follows:
Under each Social-InterestCast, a larger dissemination pattern exponent $\varphi$ leads to a smaller probability that the source chooses larger number of destinations from its friends, which leads to a lower transport load.

\begin{table*}[!t]
	\renewcommand{\arraystretch}{1.5}
	\centering
	\caption{Lower Bounds on $ \sum\nolimits_{k=1}^{n}|\mathrm{EMST}(\mathcal{P}^\mathrm{I}_k)|$}
	\label{tab-lower-bound-EMST}
	\scalebox{0.75}
	{
		%\begin{tiny}
		\begin{tabular}{|p{1.8cm}||p{3.85cm}|p{3.85cm}|p{3.85cm}|p{3.85cm}|p{3.85cm}|}
			\hline
			$\varphi$ $\backslash$ $\beta$ & $\beta>2$ & $\beta=2$ & $ 1<\beta<2 $ & $\beta=1$ & $0\leq\beta<1$ \\
			\hline
			\hline
			
			
			$\varphi>\frac{3}{2}$ &
			$ \Omega(n)$ , $\gamma\geq0$; &
			$ \Omega(n \cdot \log n)$ , $\gamma\geq0$; &
			$ \Omega(n^{2-\frac{\beta}{2}})$ , $\gamma\geq0$; &
			$ \Omega(n^{\frac{3}{2}} / \sqrt{\log n})$ , $\gamma\geq0$; &
			$ \Omega(n^{\frac{3}{2}})$ , $\gamma\geq0$. \\
			\hline
			
			$\varphi=\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\Omega(n)  ,   \\
				\qquad \gamma>1; \\
				\Omega(n \cdot \log n)  ,  \\
				\qquad 0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n \cdot \log n)  ,   \\
				\qquad \gamma>1; \\
				\Omega(n \cdot (\log n)^2)  ,  \\
				\qquad 0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{2-\frac{\beta}{2}})  ,   \\
				\qquad \gamma>1; \\
				\Omega(n^{2-\frac{\beta}{2}} \cdot \log n)  ,  \\
				\qquad 0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad \gamma>1; \\
				\Omega(n^{\frac{3}{2}} \cdot \sqrt{\log n})  ,  \\
				\qquad  0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}})  ,   \\
				\qquad \gamma>1; \\
				\Omega(n^{\frac{3}{2}} \cdot \log n)  ,  \\
				\qquad 0\leq\gamma\leq1.\\
			\end{array}
			\right. $  \\
			\hline
			
			$1<\varphi<\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\Omega(n)  ,   \\
				\qquad \gamma>\frac{5}{2}-\varphi;\\
				\Omega(n \cdot \log n) , \\
				\qquad \gamma=\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{7}{2}-\gamma-\varphi}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{5}{2}-\varphi} / \log n) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{5}{2}-\varphi})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n \cdot \log n)  ,   \\
				\qquad \gamma>\frac{5}{2}-\varphi;\\
				\Omega(n \cdot (\log n)^2) , \\
				\qquad \gamma=\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{7}{2}-\gamma-\varphi} \cdot \log n) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{5}{2}-\varphi}) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{5}{2}-\varphi} \cdot \log n)  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{2-\frac{\beta}{2}})  ,   \\
				\qquad \gamma>\frac{5}{2}-\varphi;\\
				\Omega(n^{2-\frac{\beta}{2}} \cdot \log n) , \\
				\qquad \gamma=\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{9}{2}-\gamma-\varphi-\frac{\beta}{2}}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Omega(n^{\frac{7}{2}-\varphi-\frac{\beta}{2}} / \log n) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{7}{2}-\varphi-\frac{\beta}{2}})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad \gamma>\frac{5}{2}-\varphi;\\
				\Omega(n^{\frac{3}{2}} \cdot \sqrt{\log n}) , \\
				\qquad \gamma=\frac{5}{2}-\varphi;  \\
				\Omega(n^{4-\gamma-\varphi} / \sqrt{\log n}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Omega(n^{3-\varphi} / (\log n)^{\frac{3}{2}}) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{3-\varphi} / \sqrt{\log n})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}})  ,   \\
				\qquad \gamma>\frac{5}{2}-\varphi;\\
				\Omega(n^{\frac{3}{2}} \cdot \log n) , \\
				\qquad \gamma=\frac{5}{2}-\varphi;  \\
				\Omega(n^{4-\gamma-\varphi}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Omega(n^{3-\varphi} / \log n) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{3-\varphi})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$\varphi=1$ & $\left\{
			\begin{array}{ll}
				\Omega(n)  , \\
				\qquad  \gamma\geq\frac{3}{2}; \\
				\Omega(n^{\frac{5}{2}-\gamma} / \log n) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{3}{2}} / (\log n)^2) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{3}{2}} / \log n)  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n \cdot \log n)  , \\
				\qquad  \gamma\geq\frac{3}{2}; \\
				\Omega(n^{\frac{5}{2}-\gamma}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{3}{2}} / \log n) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{3}{2}})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{2-\frac{\beta}{2}})  , \\
				\qquad  \gamma\geq\frac{3}{2}; \\
				\Omega(n^{\frac{7}{2}-\gamma-\frac{\beta}{2}} / \log n) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{5}{2}-\frac{\beta}{2}} / (\log n)^2) , \\
				\qquad \gamma=1;  \\
				\Omega(n^{\frac{5}{2}-\frac{\beta}{2}} / \log n)  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}} / \sqrt{\log n})  , \\
				\qquad  \gamma\geq\frac{3}{2}; \\
				\Omega(n^{3-\gamma} / (\log n)^{\frac{3}{2}}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{2} / (\log n)^\frac{5}{2}) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{2} / (\log n)^\frac{3}{2})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}})  , \\
				\qquad  \gamma\geq\frac{3}{2}; \\
				\Omega(n^{3-\gamma} / \log n) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Omega(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{2} / \log n)  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$0\leq\varphi<1$ & $\left\{
			\begin{array}{ll}
				\Omega(n)  , \\
				\qquad  \gamma>\frac{3}{2}; \\
				\Omega(n \cdot \log n)  , \\
				\qquad  \gamma=\frac{3}{2}; \\
				\Omega(n^{\frac{5}{2}-\gamma}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{3}{2}} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{\frac{3}{2}})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n \cdot \log n)  , \\
				\qquad  \gamma>\frac{3}{2}; \\
				\Omega(n \cdot (\log n)^2)  , \\
				\qquad  \gamma=\frac{3}{2}; \\
				\Omega(n^{\frac{5}{2}-\gamma} \cdot \log n) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{3}{2}}) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{\frac{3}{2}} \cdot \log n)  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{2-\frac{\beta}{2}})  , \\
				\qquad  \gamma>\frac{3}{2}; \\
				\Omega(n^{2-\frac{\beta}{2}} \cdot \log n)  , \\
				\qquad  \gamma=\frac{3}{2}; \\
				\Omega(n^{\frac{7}{2}-\gamma-\frac{\beta}{2}}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{\frac{5}{2}-\frac{\beta}{2}} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{\frac{5}{2}-\frac{\beta}{2}})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}} / \sqrt{\log n})  , \\
				\qquad  \gamma>\frac{3}{2}; \\
				\Omega(n^{\frac{3}{2}} \cdot \sqrt{\log n})  , \\
				\qquad  \gamma=\frac{3}{2}; \\
				\Omega(n^{3-\gamma} / \sqrt{\log n}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Omega(n^{2} / (\log n)^{\frac{3}{2}}) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{2} / \sqrt{\log n})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Omega(n^{\frac{3}{2}})  , \\
				\qquad  \gamma>\frac{3}{2}; \\
				\Omega(n^{\frac{3}{2}} \cdot \log n)  , \\
				\qquad  \gamma=\frac{3}{2}; \\
				\Omega(n^{3-\gamma}) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Omega(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Omega(n^{2})  , \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
		\end{tabular}
		%\end{tiny}
	}
\end{table*}

\begin{table*}[!t]
	\renewcommand{\arraystretch}{1.5}
	\centering
	\caption{The Order of Lower Bounds on The Derived Transport Load,  $G\left(\beta, \gamma, \varphi\right)$}
	\label{G-tab-total}
	\scalebox{0.75}
	{
		%\begin{tiny}
		\begin{tabular}{|p{1.8cm}||p{3.85cm}|p{3.85cm}|p{3.85cm}|p{3.85cm}|p{3.85cm}|}
			
			
			\hline
			$\varphi$ $\backslash$ $\beta$ & $\beta>2$ & $\beta=2$ & $ 1<\beta<2 $ & $\beta=1$ & $0\leq\beta<1$ \\
			\hline
			\hline
			
			
			$\varphi>2$ &
			$ \Theta(n) , \gamma\geq0 $ &
			$ \Theta(n \cdot \log n) , \gamma\geq0 $ &
			$ \Theta(n^{2-\frac{\beta}{2}}) , \gamma\geq0 $ &
			$ \Theta(n^{\frac{3}{2}} / \sqrt{\log n}), \gamma\geq0 $ &
			$ \Theta(n^{\frac{3}{2}}) , \gamma\geq0 $ \\
			\hline
			
			$\varphi=2$ & $\left\{
			\begin{array}{ll}
				\Theta(n)  , \\
				\qquad   \gamma >1;\\
				\Theta(n \cdot \log n) ,  \\
				%\qquad \gamma=1;  \\
				%\Theta(n \cdot \log n)  , \\
				\qquad 0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$ \Theta(n \cdot \log n) $  ,  $ \gamma\geq0. $  &
			$ \Theta(n^{2-\frac{\beta}{2}})  ,  \gamma\geq0. $  &
			$ \Theta(n^{\frac{3}{2}} / \sqrt{\log n}) $ , $ \gamma\geq0. $ &
			$ \Theta(n^{\frac{3}{2}})  ,  \gamma\geq0. $  \\
			\hline
			
			$\frac{3}{2}<\varphi<2$ & $\left\{
			\begin{array}{ll}
				\Theta(n) , \\
				\qquad  \gamma>3-\varphi;  \\
				\Theta(n \cdot \log n) , \\
				\qquad  \gamma=3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi})  , \\
				\qquad  1<\gamma<3-\varphi; \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad  \gamma=1; \\
				\Theta(n^{3-\varphi})  , \\
				\qquad  0\leq\gamma<1.
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n \cdot \log n) , \\
				\qquad  \gamma\geq3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi})  , \\
				\qquad  1<\gamma<3-\varphi; \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad  \gamma=1; \\
				\Theta(n^{3-\varphi})  , \\
				\qquad  0\leq\gamma<1.
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{2-\frac{\beta}{2}}) , \\
				\qquad  \gamma\geq3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi})  , \\
				\qquad  1<\gamma<3-\varphi; \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad  \gamma=1; \\
				\Theta(n^{3-\varphi})  , \\
				\qquad  0\leq\gamma<1.
			\end{array}
			\right. $ &
			%$\left\{
			%  \begin{array}{ll}
				%\Theta(n^{\frac{3}{2}} / \sqrt{\log n}) , \\
				%\qquad  \gamma>1; \\
				%\Theta(n^{\frac{3}{2}} / \sqrt{\log n}) , \\
				%\qquad  \gamma=1; \\
				$\Theta(n^{\frac{3}{2}} / \sqrt{\log n}) ,   \gamma\geq0. $ &
				%  \end{array}
			%\right. $
			%\left\{
			%  \begin{array}{ll}
				%\Theta(n^{\frac{3}{2}}) , \\
				%\qquad  \gamma>1; \\
				%\Theta(n^{\frac{3}{2}}) , \\
				%\qquad  \gamma=1; \\
				$ \Theta(n^{\frac{3}{2}}) ,  \gamma\geq0. $ \\
				%  \end{array}
			%\right. $ \\
			\hline
			
			$\varphi=\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\Theta(n)  ,   \\
				\qquad \gamma >\frac{3}{2};\\
				\Theta(n \cdot \log n) , \\
				\qquad \gamma=\frac{3}{2};  \\
				\Theta(n^{\frac{5}{2}-\gamma}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Theta(n^{\frac{3}{2}} / \log n) , \\
				\qquad \gamma=1;  \\
				\Theta(n^{\frac{3}{2}})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n \cdot \log n)  ,   \\
				\qquad \gamma \geq\frac{3}{2};\\
				\Theta(n^{\frac{5}{2}-\gamma}) , \\
				\qquad 1<\gamma<\frac{3}{2};  \\
				\Theta(n^{\frac{3}{2}} / \log n) , \\
				\qquad \gamma=1;  \\
				\Theta(n^{\frac{3}{2}})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{2-\frac{\beta}{2}})  ,   \\
				\qquad  \gamma \geq\frac{3}{2};\\
				\Theta(n^{\frac{5}{2}-\gamma}) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Theta(n^{\frac{3}{2}} / \log n) , \\
				\qquad \gamma=1;  \\
				\Theta(n^{\frac{3}{2}})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad  \gamma >1;\\
				%\Theta(n^{\frac{3}{2}} \cdot \sqrt{\log n})  ,  \\
				%\qquad \gamma=1; \\
				\Theta(n^{\frac{3}{2}} \cdot \sqrt{\log n})  ,  \\
				\qquad  0\leq\gamma\leq1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}})  ,   \\
				\qquad  \gamma >1;\\
				%\Theta(n^{\frac{3}{2}} \cdot \log n)  ,  \\
				%\qquad \gamma=1;\\
				\Theta(n^{\frac{3}{2}} \cdot \log n)  ,  \\
				\qquad  0\leq\gamma\leq1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$1<\varphi<\frac{3}{2}$ & $\left\{
			\begin{array}{ll}
				\Theta(n)  ,  \\
				\qquad  \gamma>3-\varphi; \\
				\Theta(n \cdot \log n) , \\
				\qquad \gamma=3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi}) , \\
				\qquad  1<\gamma<3-\varphi;  \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad  \gamma=1; \\
				\Theta(n^{3-\varphi})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n \cdot \log n)  ,  \\
				\qquad \gamma\geq3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi}) , \\
				\qquad 1<\gamma<3-\varphi;  \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad \gamma=1; \\
				\Theta(n^{3-\varphi})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{2-\frac{\beta}{2}})  ,  \\
				\qquad  \gamma\geq3-\varphi; \\
				\Theta(n^{4-\gamma-\varphi}) , \\
				\qquad  1<\gamma<3-\varphi;  \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad  \gamma=1; \\
				\Theta(n^{3-\varphi})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}} / \sqrt{\log n})  ,  \\
				\qquad \gamma>\frac{5}{2}-\varphi; \\
				\Theta(n^{\frac{3}{2}} \cdot  \sqrt{\log n}) , \\
				\qquad \gamma=\frac{5}{2}-\varphi; \\
				\Theta(n^{4-\gamma-\varphi}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad \gamma=1; \\
				\Theta(n^{3-\varphi})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}})  ,  \\
				\qquad \gamma>\frac{5}{2}-\varphi; \\
				\Theta(n^{\frac{3}{2}} \cdot \log n) , \\
				\qquad \gamma=\frac{5}{2}-\varphi; \\
				\Theta(n^{4-\gamma-\varphi}) , \\
				\qquad 1<\gamma<\frac{5}{2}-\varphi;  \\
				\Theta(n^{3-\varphi} / \log n) , \\
				\qquad \gamma=1; \\
				\Theta(n^{3-\varphi})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$\varphi=1$ & $\left\{
			\begin{array}{ll}
				\Theta(n)  ,   \\
				\qquad  \gamma\geq 2;\\
				\Theta(n^{3-\gamma} / \log n) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2} / \log n)  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n \cdot \log n)  ,   \\
				\qquad \gamma\geq 2;\\
				\Theta(n^{3-\gamma} / \log n) , \\
				\qquad 1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2} / \log n)  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{2-\frac{\beta}{2}})  ,   \\
				\qquad \gamma\geq 2;\\
				\Theta(n^{3-\gamma} / \log n) , \\
				\qquad 1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2} / \log n)  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad \gamma\geq 2;\\
				\Theta(n^{3-\gamma} / \log n) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2} / \log n)  ,  \\
				\qquad 0\leq\gamma<1.\\
				
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}})  ,   \\
				\qquad \gamma\geq 2;\\
				\Theta(n^{3-\gamma} / \log n) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / (\log n)^2) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2} / \log n)  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
			
			$0\leq\varphi<1$ & $\left\{
			\begin{array}{ll}
				\Theta(n)  ,   \\
				\qquad  \gamma>2;\\
				\Theta(n \cdot \log n) , \\
				\qquad  \gamma=2;  \\
				\Theta(n^{3-\gamma}) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2})  ,  \\
				\qquad 0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n \cdot \log n)  ,   \\
				\qquad  \gamma\geq2;\\
				\Theta(n^{3-\gamma}) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(2-\frac{\beta}{2})  ,   \\
				\qquad \gamma\geq2;\\
				\Theta(n^{3-\gamma}) , \\
				\qquad  1<\gamma<2;  \\
				\Theta(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}} / \sqrt{\log n})  ,   \\
				\qquad  \gamma>\frac{3}{2};\\
				\Theta(n^{\frac{3}{2}} \cdot \sqrt{\log n}) , \\
				\qquad  \gamma=\frac{3}{2};  \\
				\Theta(n^{3-\gamma}) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Theta(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ &
			$\left\{
			\begin{array}{ll}
				\Theta(n^{\frac{3}{2}})  ,   \\
				\qquad  \gamma>\frac{3}{2};\\
				\Theta(n^{\frac{3}{2}} \cdot \log n) , \\
				\qquad  \gamma=\frac{3}{2};  \\
				\Theta(n^{3-\gamma}) , \\
				\qquad  1<\gamma<\frac{3}{2};  \\
				\Theta(n^{2} / \log n) , \\
				\qquad  \gamma=1;  \\
				\Theta(n^{2})  ,  \\
				\qquad  0\leq\gamma<1.\\
			\end{array}
			\right. $ \\
			\hline
		\end{tabular}
		%\end{tiny}
	}
\end{table*}

==> overview.tex <==
%The overview of our proposed framework for online lending fraud detection by multi-stage data representation, named OCLFP-MS, is shown in Fig. \ref{figure:Overview}, which consists of the following components:


The workflow of our framework consists of four main parts: three representation stages, cooperatively acting as the information density booster, and one predictor, as shown in Fig. \ref{figure:overview}.
In this section, we give each part a brief introduction.









==> problem.tex <==


% ; let a subset $\mathcal{S}=\{v_{\mathcal{S},k}\}_{k=1}^{n_s} \subseteq \mathcal{V}$ denote the set of all sources, where $|\mathcal{S}|=n_s$.


